Exploring Weight Importance and Hessian Bias in Model Pruning

Model pruning is an essential procedure for building compact and computationally-efficient machine learning models. A key feature of a good pruning algorithm is that it accurately quantifies the relative importance of the model weights. While model pruning has a rich history, we still don't have a full grasp of the pruning mechanics even for relatively simple problems involving linear models or shallow neural nets. In this work, we provide a principled exploration of pruning by building on a natural notion of importance. For linear models, we show that this notion of importance is captured by covariance scaling which connects to the well-known Hessian-based pruning. We then derive asymptotic formulas that allow us to precisely compare the performance of different pruning methods. For neural networks, we demonstrate that the importance can be at odds with larger magnitudes and proper initialization is critical for magnitude-based pruning. Specifically, we identify settings in which weights become more important despite becoming smaller, which in turn leads to a catastrophic failure of magnitude-based pruning. Our results also elucidate that implicit regularization in the form of Hessian structure has a catalytic role in identifying the important weights, which dictate the pruning performance.

==> broader.tex <==
\section*{Broader Impact}

Widespread adoption of deep networks pave the way towards a future where variety of application domains benefit from artificial intelligence. However, energy and storage cost of the contemporary deep learning models are a critical bottleneck in deploying machine learning in practical setups such as mobile applications. The extremely large models and the associated computational inefficiency are also serious concerns for small businesses and research labs that cannot afford fleets of GPUs. This brings us to topic of our work. Pruning techniques are essential to overcoming these problems and building efficient models. Despite its practical impact, we unfortunately do not have a good grasp of which pruning algorithm works well and why. In practice, this may lead to wasted effort for a machine learning engineer, deployment of a suboptimal product, and bad user experience, such as high-latency, for the end user of the AI model. In this work, we develop a fundamental understanding of various algorithmic choices and explain which approach works under what condition in a principled fashion. Besides advancing state-of-the-art, we strongly believe our findings will help practitioners make more theoretically-grounded decisions.% while advancing theory.
% extreme size of many state-of-the-art deep nets is

%In this paper we develop a precise and asymptotically exact understanding of the statistical behavior of a variety of classification algorithms. In particular we precisely, characterize how the total and class-wise accuracy varies under different training algorithms, data distributions, problem dimensions, inter/intra class correlations and class priors. Despite being theoretical/foundational in nature it has potential for broader practical impact. In particular, our precise characterization of class-wise accuracy allows us to understand how different training algorithms impact accuracy of machine learning algorithms on rare/minority classes. Such a precise understanding may help guide the development of more fair/equitable algorithms. On the flip side, in the wrong hands such insights may potentially be used nefariously enabling the marginalization of rare/minority classes by developing algorithms that reduce the accuracy for certain classes.



==> covar_result.tex <==
\section{Scale-Dependence of the Overparameterized Pseudo-inverse}\label{scale dep}


%\noindent {\bf{Pseudo-inverse change:}} 
The goal of this section is demonstrating the variability of feature importance in over-parameterized least-squares by studying the effect of feature scaling. 

%Our goal is finding a model $\bt$ with small test error i.e.~for a fresh sample $(\x,y)$, $\E[(y-\bt^T\x)^2]$ is small.
Suppose we are given a dataset $\y\in\R^n$ and $\X\in\R^{n\times p}$ and assume that $\X$ is full-rank. Clearly pseudo-inverse $\hat{\bt}=\X^\dagger \y$ is a common method for finding a model $\bt$ that can predict $\y$ given $\X$. Now, let $\La\in\R^{p\times p}$ be a diagonal matrix with nonnegative diagonal entries which will be used to scale our $p$ features as follows.

Let us consider a problem with labels $\y$ and scaled input features $\X\sqrt{\La}$. In this case, an alternative model that can predict $\y$ given unscaled $\X$ can be obtained by solving pseudo-inverse on the scaled problem $(\y,\X\sqrt{\La})$ and multiplying the solution by $\sqrt{\La}$ to account for the scaling. This model is given by
\[
\hat{\bt}_{\La}=\sqrt{\La}(\X\sqrt{\La})^\dagger \y.
\]
%Alternatively, one can estimate $\bt$ by solving the problem with labels $\y$ and inputs $\X\sqrt{\La}$. %Now  $\X$ is scaled with a diagonal matrix $\La^{1/2}$, we have the pair 
It is a simple exercise to show that if the problem is under-parameterized ($n\geq p$), $\hat{\bt}_{\La}$ is independent of scaling $\La$ and is always equal to the true pseudo-inverse $\hat\bt=\X^T(\X\X^T)^{-1}\y$. However if the problem is over-parameterized, $\hat{\bt}_{\La}$ has $\La$ dependence and is given by
\begin{align*}
\hat{\bt}_{\La}&=\sqrt{\La}(\X\sqrt{\La})^\dagger \y=\sqrt{\La}(\sqrt{\La}\X^T(\X\La\X^T)^{-1}\y)\\
&=\La\X^T(\X\La\X^T)^{-1}\y.
\end{align*}
Following this observation, we will show that as a feature weight increases (i.e.~diagonal entry of $\La$ associated to that feature), the model weight (the corresponding entry of $\hat{\bt}_{\La}$) increases as well. The following lemma summarizes this by focusing on scaling the first feature (without losing generality). 

\mli{inf data, $\theta$ iid, linear $y=x\theta$, solve $diag(\Lambda)x$, doesn't change test. finite data ... + feature scaling $\theta$ changes, connect to loss}

%\begin{lemma}[Feature scaling in linear regression] Suppose $p>n$. Let $\La=\text{diag}([\la~1~1~\dots~1])$. Given $\X,\y$ consider the scaled pseudo-inverse model defined as $\hat{\bt}_{\la}:=\hat{\bt}_{\La}$. Let $\x$ be the first column of $\X$. Suppose remaining $p-1$ columns of $\X$ have full row-rank and define their inverse gram matrix as $\Cb=(\X\X^T-\x\x^T)^{-1}$. The first entry of $\hat{\bt}_{\la}$ is given by
%\[
%\hat{\bt}_{\la,1}=\frac{\x^T\Cb\y}{\la^{-1}+\x^T\Cb\x}.
%\]
%
%
%
%\end{lemma}
%As $\la$ increases from $0$ to $\infty$, $\hat{\bt}_{\la,1}$ moves from $0$ to $\frac{\x^T\Cb\y}{\x^T\Cb\x}$. Specifically, the model weight $|\hat{\bt}_{\la,1}|$ of the first feature is a strictly increasing function of $\la\geq 0$ whenever $\x^T\Cb\y\neq 0$.
%
%\begin{proof}
%%Let $\y=\X\eb_1$. We have $\hat\bt=\X^\dagger \y=\X^T(\X\X^T)^{-1}\y$. The solution of $\X\sqrt{\La}$ is given by . Then $\hat{\eb}_1=\La^{1/2}\hat\bt=\La\X^T(\X\La\X^T)^{-1}\y$.
%%\[
%%\X\La\X^T=\sum_{i=1}^p \la_i\x_i\x_i^T.
%%\]
%%In the extreme case of $n=1$, $\hat{\eb}_1$ is strictly increasing function of the entries of $\La$. What about matrix inversion lemma for more general case?
%Set $\Cb=(\X_-\X_-^T)^{-1}$. Note that $\X\sqrt{\la}(\X\sqrt{\la})^T=\Cb^{-1}+\la\x\x^T$. Let us apply Matrix Inversion Lemma to obtain
%\[
%(\X\La \X^T)^{-1}=\Cb-(\la^{-1}+\x^T\Cb\x)^{-1}\Cb\x\x^T\Cb
%\]
%Hence
%\[
%(\X\La \X^T)^{-1}\y=(\Iden-(\la^{-1}+\x^T\Cb\x)^{-1}\Cb\x\x^T)\Cb\y.
%\]
%%\[
%%\frac{\la_i x_i}{\sum_{i=1}^p \la_ix_i^2}
%%\]
%Consequently, the first entry of $\La\X^T(\X\La \X^T)^{-1}\y$ is given by
%\begin{align*}
%\hat{\bt}_{\la,1}&=\la\x^T(\Iden-(\la^{-1}+\x^T\Cb\x)^{-1}\Cb\x\x^T)\Cb\y\\
%&=\la\x^T\Cb\y(1-\frac{\x^T\Cb\x}{\la^{-1}+\x^T\Cb\x})\\
%&=\la\x^T\Cb\y(\frac{\la^{-1}}{\la^{-1}+\x^T\Cb\x})\\
%&=\frac{\x^T\Cb\y}{\la^{-1}+\x^T\Cb\x}.
%%\\&\la-\la(\la^{-1}+\x^T\Cb^{-1}\x)^{-1}\x^T\Cb^{-1}\x=\la(1-\frac{\alpha}{\la^{-1}+\alpha})=\frac{1}{\la^{-1}+\alpha}
%\end{align*}
%Note that $\lim_{\la\rightarrow 0}\hat{\bt}_{\la,1}=0$ and $\hat{\bt}_{\infty,1}=\frac{\x^T\Cb\y}{\x^T\Cb\x}$.
%%Differentiating, we find that feature weight is a strictly increasing function of $\la$.
%\end{proof}


%\[
%1-\frac{\alpha}{}
%\]
%Now, set $\bar{\x}=\La^{-1/2}\x$ and let us study a single gradient iteration. Observe that
%\begin{align}
%\h=\X^T\y=\La^{1/2}\bar{\X}^T\X\bt=\La^{1/2}\bar{\X}^T\bar{\X}\bar{\bt}.
%\end{align}
%\begin{align}
%\h&=\X^\dagger\y=\X^T(\X\X^T)^{-1}\y=\La^{1/2}\bar{\X}^T(\bar{\X}\La\bar{\X}^T)^{-1}\bar{\X}\bar{\bt}\\
%&=\X^\dagger\y=(\X^T\X)^{-1}\X^T\y=(\La^{1/2}\bar{\X}\bar{\X}^T\La^{1/2})^{-1}\La^{1/2}\bar{\X}^T\bar{\X}\bar{\bt}
%\end{align}
%\[
%\h=\X^T\y=\sum_{i=1}^n y_i\x_i=\sum_{i=1}^n \x_i\x_i^T\bt=\sum_{i=1}^n \La^{1/2}\xb_i\xb_i^T\bar{\bt}.
%\]
%Hence
%\begin{align}
%h_j&=\sqrt{\la}_j\sum_{i=1}^n \bar{x}_{i,j}\xb_i^T\bar{\bt}\\
%&=\sqrt{\la}_j(\bar{\theta}_j +\bar{\theta}_j (\bar{x}_{i,j}^2-1)+\bar{x}_{i,j}\xb_{i,\neq j}^T\bar{\bt}_{i,\neq j})
%%=\sqrt{\la}_j\theta_j+\sum_{i=1}^n\sqrt{\la_i\la_j}\theta_i.
%\end{align}
%Select most predictive features i.e. $\gamma$ fraction of the overall energy.

%\begin{lemma}[Shrinkage lemma] Let $\bt_\st$ be an $s$-sparse vector and suppose $\bt'=\bt_\st+\ab+\bb$ where $\tin{\bb}\leq \gamma$. Then for $\la\geq \gamma$, $\hat{\bt}=\prox{\la}(\bt')$ obeys $\tn{\hat{\bt}-\bt_\st}\leq \tn{\ab}+2\sqrt{s}\la$.
%\end{lemma}
%\begin{proof} Let $S$ be the support of $\bt_\st$. For $i\in S$, we have that
%\[
%|\shr{\la}{\bt_\st[i]+\ab[i]+\bb[i]}-\bt_\st[i]|\leq |\ab[i]|+|\bb[i]|+\la\leq  |\ab[i]|+2\la.
%\]
%For $i\in S^c$, we have
%\[
%|\shr{\la}{\ab[i]+\bb[i]}|\leq \max(0,|\ab[i]|+|\bb[i]|-\la)\leq  |\ab[i]|.
%\]
%Combining these, we find the desired result.
%\end{proof}


==> deter_result.tex <==

%\section{Main Results}
\section{Feature Selection via Gradient Descent}\label{improve feature sec}
%\begin{figure}[t!]
%	\begin{subfigure}{2.6in}
%		\begin{tikzpicture}[scale=1.1,every node/.style={scale=1.1}]
%		\node at (0,0) {\includegraphics[scale=0.38]{figs/pruning_jacobian_bn}};
%		\node at (-3,0) [rotate=90,scale=.8]{Accuracy};
%		\node at (0,-2.1) [scale=.8]{Non-zero level};
%		\end{tikzpicture}\caption{Test accuracy on 4 pruning methods when using batch normalization}\label{fig:jacobian_bn}
%	\end{subfigure}
%	\begin{subfigure}{2.6in}
%	\begin{tikzpicture}[scale=1.1,every node/.style={scale=1.1}]
%	\node at (0,0) {\includegraphics[scale=0.38]{figs/pruning_jacobian_nobn}};
%	\node at (-3,0) [rotate=90,scale=.8]{Accuracy};
%	\node at (0,-2.1) [scale=.8]{Non-zero level};
%	\end{tikzpicture}\caption{Test accuracy on 4 pruning methods without using batch normalization}\label{fig:jacobian_nobn}
%\end{subfigure}
%\end{figure}
%\begin{figure}[t!]
%	\begin{subfigure}{1.8in}
%		\begin{tikzpicture}[scale=0.8,every node/.style={scale=0.8}]
%		\node at (0,0) {\includegraphics[scale=0.38]{figs/gradient_norm}};
%		\node at (-3,0) [rotate=90,scale=.8]{$\tn{m\odot\nabla\Lc(\bt_\tau)}^2$};
%		\node at (0,-2.1) [scale=.8]{Epoch};
%		\end{tikzpicture}\caption{Gradient energy of bottom vs top entries.}\label{fig:gradient_norm}
%	\end{subfigure}
%	\begin{subfigure}{1.8in}
%		\begin{tikzpicture}[scale=0.8,every node/.style={scale=0.8}]
%		\node at (0,0) {\includegraphics[scale=0.38]{figs/gradient_fraction}};
%		\node at (-3,0) [rotate=90,scale=.8]{Fraction of masked gradient};
%		\node at (0,-2.1) [scale=.8]{Epoch};
%		\end{tikzpicture}\caption{Fraction of the top/bottom gradient energy}\label{fig:gradient_fraction} 
%	\end{subfigure}
%	\begin{subfigure}{1.8in}
%		\begin{tikzpicture}[scale=0.8,every node/.style={scale=0.8}]
%		\node at (0,0) {\includegraphics[scale=0.38]{figs/energy_fraction}};
%		\node at (-3,0) [rotate=90,scale=.8]{Fraction of masked weight};
%		\node at (0,-2.1) [scale=.8]{Epoch};
%		\end{tikzpicture}\caption{Fraction of the top/bottom weight energy.}\label{fig:weight_fraction} 
%	\end{subfigure}
%	\caption{We select $\text{mask}^{10\%}_{top}(\bar{\bt}_{final})$ $\text{mask}^{10\%}_{btm}(\bar{\bt}_{final})$ which are the top and bottom 10\% entries of the final weight distances $\bar{\bt}_{final}=\bt_{final}-\bt_{0}$ (per Def.~\ref{def:mask}). Each layer is treated individually and keeps $10\%$ of the entries. We train 10 class ResNet-20 with CIFAR-10 without data augmentation, compute the full gradient of train and test datasets and plot the evolution of the top/bottom 10\% of the gradient. Fig.~\ref{fig:gradient_norm} shows the energy $\tn{m\odot\nabla\Lc(\bt_\tau)}^2$ of top and bottom for all epochs for both test and training data. Fig.~\ref{fig:gradient_fraction} shows the fraction of the top/bottom of the full gradient. The gradient of the top distances are consistently larger during the training. Fig.~\ref{fig:weight_fraction} shows the fraction $\tn{\text{mask}^{10\%}_{top/btm}(\bar{\bt}_{\tau})}^2/\tn{\bar{\bt}_{\tau}}^2$ for the top/bottom of the weight moving distance where $\bar{\bt}_{\tau}=\bt_\tau-\bt_0$.\\
%%	\com{Highlight that there is significant difference between distance and weight pruning!}\\
%%	\com{Explain why lottery ticket is better than our experiments e.g.~layer-targeted pruning, regularization, data augment etc. For CIFAR10 try to replicate lottery experiments' setup.}
%}
%	% but gradient of bottom entries vanishes after a few epoch
%	\label{fig:gradient} \vspace{-0.2cm}
%	% ($m\odot\nabla\Lc(\bt_\tau)$)
%\end{figure}
%
%\begin{figure*}[t!]
%	\begin{subfigure}{2.8in}
%		\begin{tikzpicture}[scale=1,every node/.style={scale=1}]
%		\node at (0,0) {\includegraphics[scale=0.38]{figs/acc_prun_top_C10_1}};
%		\node at (-3,0) [rotate=90,scale=.8]{Test accuracy};
%		\node at (0,-2.1) [scale=.8]{Fraction of non-zero};
%		\end{tikzpicture}\caption{Test accuracy when masking top entries and setting others to 0. }\label{fig:compare_purining_C10_1}
%	\end{subfigure}
%	\begin{subfigure}{2.8in}
%		\begin{tikzpicture}[scale=1,every node/.style={scale=1}]
%		\node at (0,0) {\includegraphics[scale=0.38]{figs/acc_prun_top_C10_2}};
%		\node at (-3,0) [rotate=90,scale=.8]{Test accuracy};
%		\node at (0,-2.1) [scale=.8]{Fraction of non-zero};
%		\end{tikzpicture}\caption{Test accuracy when masking top entries and setting others to initialization.}\label{fig:compare_purining_C10_2} 
%	\end{subfigure}
%	\caption{In Fig.~\ref{fig:compare_purining_C10}, we investigate combinations of two masking methods and two weight resetting methods on CIFAR10 training on ResNet-20 with softmax activation and cross-entropy loss. Let us use \textit{distance pruning} $m_{distance}^p=\text{mask}^p(\bt_{final}-\bt_0)$ to denote the pruning method that masks weight by its moving distance while training. And use \textit{weight pruning} to denote the pruning method that only considers the top entries of final weight ($m_{weight}^p=\text{mask}^p(\bt_{final})$). In Fig.~\ref{fig:compare_purining_C10_1}, we firstly mask the final weight by both pruning methods and then set other entries to 0. The solid lines show the test accuracy after masking and resetting, and the dash lines show the test accuracy after retraining on masked entries. Fig.~\ref{fig:compare_purining_C10_2} shows the test accuracy when resetting unmasked entries to their initialization after distance or weight pruning. }\label{fig:compare_purining_C10} 
%\end{figure*}

%Define the soft-thresholding operator as
%\[
%\prox{\la}(\x)=\arg\min_{\x'} \frac{1}{2}\tn{\x-\x'}^2+\la \tone{\x'}
%\]
This section will explore the properties of plain gradient descent (without explicit regularization) and investigate whether gradient descent can provably select important features in the data by leveraging the latent problem structure. Given a learning rate $\eta>0$, starting from an initial point $\bt_{\text{init}}=\bt_0$, we run gradient descent for $T$ iterations 
\begin{align}
\bt_{\tau+1}=\bt_\tau-\eta \grad{\bt_\tau}.\label{GD}
\end{align}
We then investigate the properties of the final model $\bt_{\text{final}}=\bt_T$ by studying the distance vector $\bar{\bt}_{\text{final}}=\bt_{\text{final}}-\bt_0$ with an emphasis on understanding the importance of individual weights. To explain the experiments, let us also introduce the mask function for pruning.% or weight groups.% its larger/smaller coordinates.% in different ways.% focusing on which weights are more important than others.
%for $T$ iterations and study $\bt_T$.%implicit structure in the design matrix. 



%\begin{definition}[Mask function]
%	\mli{Do I need it?}
%	Given model $f(\x,\bt)$ with weights $\bt\in\R^d$, a mask is a function satisfying $$\text{mask}^p(\bt): \R^{d} \to \{0,1\}^{d}$$ such that $0\leq p\leq 1$ fraction of the $d$ entries in $\text{mask}^p(\bt)$ are equal to 1. Mask can be used to prune the weights $\bt$ via $\text{mask}^p(\bt)\odot\bt$ where $\odot$ returns the entrywise product.% where $m=$.
%	\label{def:mask}
%	
%\end{definition}

\subsection{Stronger Feature Wins More}
%As a starting point of our discussion, consider the following toy example: We wish to fit an overparameterized least-squares problem \eqref{LS} where there are two groups of features so that the design matrix $\X$ can be written as $\X=[\X_1~\X_2]$ where $\X_1\in\R^{n\times p_1}$ and $\X_2\in\R^{n\times p_2}$. Splitting $\bt$ into two groups as well, we minimize
%\begin{align}
%\min_{\bt}\Lc(\bt)\quad\text{where}\quad \bt=[{\bt^{(1)}}^T~{\bt^{(2)}}^T]^T.\label{bt split}
%\end{align}
where $\Lc(\bt)=\frac{1}{2} \tn{\y-\X_1\bt^{(1)}-\X_2\bt^{(2)}}^2$. Suppose both feature groups are large so that $p_1\wedge p_2\geq n$ and $\X_1$ and $\X_2$ are full row-rank. Under this circumstances, clearly $\X_1$ and $\X_2$ can both perfectly fit to the labels $\y$ which is a common scenario in overparameterized problems. The natural question for us is what are the properties of the gradient-based solution? An intuitive solution is ``May the feature with larger gradient win''. In consistence with the pruning literature, Figure \ref{fig:gradient} shows that there are indeed strong and weak weights in deep networks. The largest/smallest weights found at the end of the training are consistently so throughout the training. The blue solid line in Fig.~\ref{fig:compare_purining_C10_2} shows that when masking the weight with largest movement in training and reset others to initialization, the masked network achieves highest test accuracy among multiple mask method. Perhaps surprisingly, this observation continues to hold on the gradient over the test data. Below we formalize the ``stronger wins more'' intuition.

Earlier works \cite{du2019gradient,oymak2019overparameterized} show that gradient descent on quadratic loss has preference towards minimum distance (or norm) solutions. Thus, we can expect that gradient descent will prefer the feature group that can lead to a shorter distance. In other words, it will prefer the feature group that can explain the labels $\y$ as fast as possible. Naturally, pace of explanation is related to the size of the gradient at a particular feature. Our first theorem establishes an optimization result by making this idea rigorous for loss functions with Lipschitz gradients satisfying the Polyak-Lojasiewicz (PL) inequality. PL is a common assumption in the analysis of nonconvex problems \cite{karimi2016linear}. The following result shows that stronger features (or the associated weights) can dominate the weaker ones when trained with gradient descent. Below we setup the problem so that $\bt^{(2)}$ is the weaker weights which is captured by the Lipschitz constant of the partial derivative.% The result applies to loss functions .

\som{Define partial polyak condition with respect to a set of parameters}


\som{include linear simulation if space}

The main message of the theorem above is most visible when we let $\tau\rightarrow \infty$ and when the PL growth parameter $\mu$ dominates the Lipschitz constant of $\bt^{(2)}$ i.e.~$\mu/L_2=\kappa^{-1}\gg 1$. Under this condition, removing the progress made by $\bt^{(2)}$ (by setting $\bt^{(2)}_\tau$ to $\bt^{(2)}_0$) only mildly hurts the performance as the loss is at most $8\kappa \Lc(\bt_0)$. In contrast, focusing only on $\bt^{(2)}$ by removing the contribution of $\bt^{(1)}$ demonstrates that $\bt^{(2)}$ itself only reduces the loss proportional to $\sqrt{\kappa}$. Our proof strategy builds on \cite{oymak2019overparameterized,gupta2019path} which establish distance bounds for solutions found by gradient descent. Our result is consistent with Figure \ref{fig:bin_neuralnet_accuracy}. Neural network is more resilient to keeping the top distance weights and removing the bottom distance weights (pruning weaker features). Supplementary material shows that our theorem perform best among different pruning strategies and provides further experiments (e.g.~by weights, distance, setting to $0$).% theExperiments where we go back to $\ material provides further numerical results %However accuracy is extremely sensitive to the removal of random weights (which ends up removing the important weights as well).%
%  sets the loss approximately to its initial state i.e.~

Going back to the least-squares problem \eqref{LS}, suppose $\X_2$ is weaker than $\X_1$ in the sense that $\sigma_{\min}(\X_1)\gg \|\X_2\|$. This implies $\mu\gg L_2$, since for linear regression \eqref{LS}, it can be shown that, $\mu =\sigma^2_{\min}(\X)\geq \sigma^2_{\min}(\X_1)$ and $L_2=\|\X_2\|^2$. Thus, gradient descent will prefer $\X_1$ over $\X_2$ and most of the prediction of the final model will be due to $\X_1$. While Theorem \ref{lem small grad} considers possibly non-convex problems, Appendix C provides further insights on how modifying the feature strength via scaling affect the solutions of the linear problem \eqref{LS}.%monotonic behavior of fe

% when data $(\x_i,y_i)_{i=1}^n$ is drawn i.i.d.~from a distribution
While Theorem \ref{lem small grad} is an optimization result, finding nearby solutions is inherently connected to generalization via Rademacher complexity arguments \cite{bartlett2002rademacher}. Additionally, one would expect that important parameter weights (with larger gradients) should be learnable with fewer samples. For linear models, large gradient is associated to the larger correlation between label and features i.e.~$\frac{\pa \Lc(\bt)}{\pa \bt_i}\approx\E[x_{i}y]$. Such intuitions appear in neural network pruning as well as earlier seminal algorithms such as Orthogonal Matching Pursuit and CoSaMP among others \cite{needell2008cosamp,tropp2007signal}. Focusing on single index models where data is generated as $y=\phi(\x^T\bt)$ for some unknown link function $\phi$, in Appendix B, we establish feature-strength dependent sample bounds and exemplify how stronger features are learnable from fewer samples.% rigorizes the 


% of indi instance, when data $(\x_i,y_i)_{i=1}^n$ is drawn i.i.d.~from a distribution, intuitively features with larger gradient (e.g.~   are one would expect that stronger features can be discovered from  We also remark that Feature strength  short distance Indeed, correlation between the feature and gradient is a proxy for seminal compressed sensing literature such as \cite{} leverages related ideas.






%Thus, focusing on quadratic loss $\Lc(\bt)=\tn{\y-\X\bt}^2/2$, we study the following two stage estimator starting from an initial model $\bt_0$.% We will focus on first order methods to estimate important features induced by $\bt_\st$. As a proxy for lasso regression, starting from $\bt_0=0$, our estimation procedure is as follows.

%In contrast to iterative soft/hard-thresholding which occurs at every iteration \cite{}, we only carry out the thresholding at the very end to select the prominent features. We also remark that gradient descent with early-stopping is connected to the ridge regression \cite{}. 


%\begin{figure*}[t!]
%	\begin{subfigure}{2.1in}
%		\begin{tikzpicture}[scale=0.9,every node/.style={scale=0.9}]
%		\node at (0,0) {\includegraphics[scale=0.38]{figs//theory_pruning/correlation_acc}};
%		\node at (-3,0) [rotate=90,scale=.8]{Test accuracy};
%		\node at (0,-2.1) [scale=.8]{Fraction of non-zero};
%		\end{tikzpicture}\caption{Test accuracy on multiple masking level \\ \quad}\label{fig:bin_neuralnet_accuracy}
%	\end{subfigure}
%	\begin{subfigure}{2.1in}
%		\begin{tikzpicture}[scale=0.9,every node/.style={scale=0.9}]
%		\node at (0,0) {\includegraphics[scale=0.38]{figs/theory_pruning/correlation_zm}};
%		\node at (-3,0) [rotate=90,scale=.8]{Jacobian Correlation};
%		\node at (0,-2.1) [scale=.8]{Fraction of non-zero};
%		\end{tikzpicture}\caption{Correlation between the weights and the Jacobian matrix for varying level of masking.}\label{fig:bin_neuralnet_correlation} 
%	\end{subfigure}
%	\begin{subfigure}{2.1in}
%		\begin{tikzpicture}[scale=0.9,every node/.style={scale=0.9}]
%		\node at (0,0) {\includegraphics[scale=0.38]{figs/theory_pruning/spectrum_mean}};
%		\node at (-3,0) [rotate=90,scale=.8]{Normalized singular value};
%		\node at (0,-2.1) [scale=.8]{Index of singular value};
%		\end{tikzpicture}\caption{Jacobian spectrum and correlation of the distance vector $\bar{\bt}_{final}$ with the Jacobian}\label{fig:bin_neuralnet_spectrum} 
%	\end{subfigure}
%	\caption{Comparison of two weight masking methods (random vs larger distance). We train binary ResNet-20 with quadratic loss on five pairs of classes on CIFAR-10 (e.g. airplane vs automobile, bird vs cat) and mask by the distances $\bar{\bt}_{final}=\bt_{final}-\bt_0$. For the green and orange lines, we mask top and bottom $p\%$ entries using $m_{top/bottom}^p=\text{mask}^p(\bar{\bt}_{\text{final}})$ (per Def.~\ref{def:mask}) where $p$ is the nonzero fraction in the x-axis. Then we mask final weight entries and set other entries to their initial values per Thm.~\ref{lem small grad} as $\bt_{final}^{prune}=m_{top}^p\odot\bt_{final}+(\mathds{1}-m_{top}^p)\odot\bt_{0}$. To compare, the same fraction of random entries are masked in blue lines, using random mask $m_{rnd}^p$. The solid line in Fig.~\ref{fig:bin_neuralnet_accuracy} shows the test/train accuracy when we only use the masked network to predict. Then we retrain the initial weights $\bt_{0}$ with mask $m^p$ which only update gradient  $\nabla\Lc_{masked}=m^p\odot\nabla\Lc$ on masked entries and report the test accuracy in the dashed line in Fig.~\ref{fig:bin_neuralnet_accuracy}. We note that pruning top keeps high accuracy even without retrain and achieves just slight degradation after retraining at $10\%$ masking compared to full network. Fig.~\ref{fig:bin_neuralnet_correlation} shows the correlation between the distances $\bar{\bt}^{\text{prune}}_{final}=m^{p}_{top}\odot(\bar{\bt}_{final})$ and the column-debaised Jacobian feature map $\bar{\Jb}=\Jb-\onebb_n\onebb_n^\top\Jb/n$ which governs the instantaneous optimization dynamics. Specifically, we plot $\tn{\bar{\Jb}\bar{\bt}^{\text{prune}}_{final}}/(\|\bar{\Jb}\|\tn{\bar{\bt}^{\text{prune}}_{final}})$ for initial and final Jacobian map and different pruning levels and strategies. The green lines (top mask) show consistently higher correlation and accuracy. In words, top weights are more important for accuracy and are better aligned with the principal eigendirections of the Jacobian. All curves are averaged over 5 datasets.}\label{fig:bin_neuralnet} \vspace{-0.3cm}
%\end{figure*}
%
%\begin{figure*}[t!]
%	\begin{subfigure}{3.2in}
%		\begin{tikzpicture}[scale=1.4,every node/.style={scale=1.4}]
%		\node at (0,0) {\includegraphics[scale=0.38]{figs/compare_pruning_set0/acc_prun_top}};
%		\node at (-3,0) [rotate=90,scale=.8]{Test accuracy};
%		\node at (0,-2.1) [scale=.8]{Fraction of non-zero};
%		\end{tikzpicture}\caption{Test accuracy when masking top entries and setting others to 0. }\label{fig:compare_purining_set0}
%	\end{subfigure}
%	\begin{subfigure}{3.2in}
%		\begin{tikzpicture}[scale=1.4,every node/.style={scale=1.4}]
%		\node at (0,0) {\includegraphics[scale=0.38]{figs/compare_pruning_setinit/acc_prun_top}};
%		\node at (-3,0) [rotate=90,scale=.8]{Test accuracy};
%		\node at (0,-2.1) [scale=.8]{Fraction of non-zero};
%		\end{tikzpicture}\caption{Test accuracy when masking top entries and setting others to initialization.}\label{fig:compare_purining_setinit} 
%	\end{subfigure}
%	\caption{In Fig.~\ref{fig:compare_purining}, we investigate combinations of two masking methods and two weight resetting methods on five classes pairs of CIFAR10 training on binary ResNet-20 with quadratic loss. Let us use \textit{distance pruning} $m_{distance}^p=\text{mask}^p(\bt_{final}-\bt_0)$ to denote the pruning method that masks weight by its moving distance while training. And use \textit{weight pruning} to denote the pruning method that only considers the top entries of final weight ($m_{weight}^p=\text{mask}^p(\bt_{final})$). In Fig.~\ref{fig:compare_purining_set0}, we firstly mask the final weight by both pruning methods and then set other entries to 0. The solid lines show the test accuracy after masking and resetting, and the dash lines show the test accuracy after retraining on masked entries. Fig.~\ref{fig:compare_purining_setinit} shows the test accuracy when resetting unmasked entries to their initialization after distance or weight pruning.}\label{fig:compare_purining} 
%\end{figure*}

%For the rest of the discussion, we assume left singular values of $\X$ is the identity matrix i.e.~$\X=\sum_{i=1}^n \sqrt{\la_i}\eb_i\vb_i^T$. This will simplify the notation however doesn't affect the generality of the results as algorithm returns the exact same answer for both $(\X,\y,\z)$ and $(\X',\y',\z')=(\Ub^T\X,\Ub^T\y,\Ub^T\z)$ triplets as inputs. Results for $(\X,\y,\z)$ can be obtained from $(\Vb^T\X,\Vb^T\y,\Vb^T\z)$ and picking $\Vb$ to be the left singular vectors of $\X$.

%
%\subsection{Spectral Bias in Gradient-Based Feature Selection} \label{sec grad cov select}
%So far, we discussed how stronger features can win more, however the exact source of the feature strength remains vague. In this section, we focus on least-squares problems and identify spectral structure of the design matrix as a source of the feature selection bias. Our starting point is Figure \ref{fig:bin_neuralnet_correlation} which shows that the weights learned by a neural network is aligned with principal directions of the Jacobian feature matrix. Table \ref{table:sparsity_level} of Section \ref{sec exp} provides further evidence towards spectral bias in elastic net optimization. To explain Figure \ref{fig:bin_neuralnet_correlation}, suppose we have a neural network $f(\x,\bt)\rightarrow\hat{y}$ with weights $\bt\in\R^p$. We set the model output $f(\bt)\in\R^n$ and consider the quadratic loss as follows
%\begin{align*}
%&\Lc(\bt)=0.5\tn{\y-f(\bt)}^2\quad\text{where}\quad f(\bt)=[f(\x_1,\bt)~\dots~f(\x_n,\bt)]^T.
%\end{align*}
%
%\mli{Move jacobian part to setup and remove the $\bar{\Jb}=\Jb-\mathds{1}_n\mathds{1^\top}_n\Jb/n$ part, Consistent with hissian, H is equal to dJ =XTX, least square, global minima. }
%
%Recent optimization literature works on deep networks \cite{jacot2018neural,su2019learning,du2019gradient,chizat2019lazy,oymak2019towards,zou2018stochastic} establishes that Jacobian feature map $\Jb(\bt)=\frac{\pa f(\bt)}{\pa \bt}\in\R^{n\times p}$ act as an ``instantaneous'' design matrix and governs the optimization dynamics via the first order approximation
%\begin{align}
%f(\bt+\Delta)\approx f(\bt)+\Jb(\bt)\Delta.\label{nn jacob}
%\end{align}
%%This approximation is at the core of the recent works on Neural Tangent Kernel. 
%Hence, properties of $\Jb$ may dictate which weights have a stronger say in the network's decision than others. However, top singular vector of original $\Jb$ can be affected by the mean of each feature, which is uninformative especially when it is an all-one vector in some cases.  We define column-debiased $\bar{\Jb}=\Jb-\mathds{1}_n\mathds{1^\top}_n\Jb/n$ where $\mathds{1}_n$ is all 1 n-dimensional vector. Thus, computing correlation on $\bar{\Jb}$ which has zero mean on each column mitigates the affection of the bias on top singular vector.
%%\begin{align}
%%\Jb_{mean}=\frac{1}{n}\sum_{i=1}^{n}{\frac{\partial f(\x_i,\bt)}{\partial \bt}} \quad \text{and} \quad \bar{\Jb}=[\frac{\partial f(\x_1,\bt)}{\partial \bt}-\Jb_{mean}~\dots~\frac{\partial f(\x_n,\bt)}{\partial \bt}-\Jb_{mean}]^T. \label{zm jacob}
%%\end{align}
%
%Figure \ref{fig:bin_neuralnet_correlation} plots the correlation between column-normalized Jacobian and the distances $\bt_{\text{final}}-\bt_{0}$ and demonstrates that the top weights have a larger alignment with the eigenspectrum of the Jacobian compared to random weights. This alignment is consistent for final Jacobian computed at the end of the training as well as the initial one (i.e.~computed with random weights). As we focus on fewer weights correlation of the random weights drop whereas top weights remain strong (i.e.~green vs blue lines).
%%. Here, we train the neural network with SGD and model starts
%%(i.e.~final representation learned by the network) compared to 
%
%
%This indicates that spectral properties of feature matrix has a critical role in pruning in neural networks. We note that the spectral bias of neural networks has been the topic of several works \cite{sagun2017empirical,pennington2018emergence,papyan2018full} however our observations target the pruning aspect. We will next provide theoretical intuitions on why gradient descent can select robust features via spectral bias without any regularization. Instead of neural networks, let us focus on overparameterized linear regression \eqref{LS} formulation as a proxy for the linearized neural network dynamics \eqref{nn jacob}.% This corresponds to the setup where Jacobian map is constant (i.e.~when network is infinitely wide and NTK approximation 
%
%
%Recall that gradient descent on linear regression converges to the solution with the minimum distance from the point of initialization. Hence, if this solution happens to be sparse (i.e.~few large weights), gradient descent will find a sparse model. The problem is that the minimum distance solution can be extremely brittle especially when the eigenspectrum is ill-conditioned as in Figure \ref{fig:bin_neuralnet_spectrum}. This is precisely why spectral bias in the problem is critical for robust identification of individual features/weights. Indeed, Fig.~\ref{fig:bin_neuralnet_spectrum} shows that the weights learned by the network (dashed lines) lie close to the top of the Jacobian spectrum. Following this, we will study robustness of feature selection when the labels $\y$ are aligned with the principle eigendirections i.e.~target function lies on the principal subspace. To state our result, we need to define the spectrum and coherence of the design matrix.% The first one captures the approximate rank of the feature covariance.
%%Several works generalized this observation to other loss functions or nonlinear models and there is a growing understanding that gradient based methods are biased towards low-complexity solutions \cite{}.  % with the sparse solution, This can happen if the miniSuppose the label vector $\y$ exactly lies on the range of $d$ left singular vectors of the design matrix $\X$.
%\begin{definition}[$(d,R,r)$-covariance spectrum] \label{def cov} Let the design matrix $\X\in\R^{n\times p}$ have singular value decomposition $\X=\Ub\sqrt{\La}\V^T=\sum_{i=1}^n\sqrt{\la_i}\ub_i\vb_i^T$ where eigenvalues $(\la_i)_{i=1}^n$ are non-increasing. Define the covariance $\bSi=\X^T\X=\sum_{i=1}^p \la_i\ub_i\ub_i^T$. Fix an integer $d$ and a scalar $R\geq 1$. Define the approximate rank $r=r(d,R)$ to be the largest integer such that $\la_r\geq {\la_d}/{R}>\la_{r+1}$ ($r\leq p$).% Define the principal subspace induced by $\ab,R$ as $\Sc_{\ab,R}=\rg{(\ub_i)_{i=1}^d}$.
%\end{definition}
%%In our theorems, we will additionally require that our choice of $\ab$ lies on the principal subspace $\Sc_{\ab,R}$.
%
%%\underset{\vb\in S}{\sup}
%\vspace{-6pt}
%\begin{definition}[$\mu$-coherence] Given a subspace $S$, define the coherence of $S$ to be $\mu(S)=\sup_{\vb\in S}~\tin{\vb}/\tn{\vb}$. Define coherence of a matrix $\Ub$ as $\mu(\Ub)=\mu(\text{range}(\Ub))$
%\end{definition}
%%\begin{definition}[$\Gamma$-approximate sparse] A vector $\bt$ is called $\Gamma$-approximate sparse if all entries obey $|\theta_i|\geq 2\Gamma$ or $|\theta_i|\leq \Gamma/2$. 
%%\end{definition}
%
%Our guarantees will be stated in terms of the support and confusion set defined below as a function of a threshold $\Gamma$.\vspace{-3pt}
%\begin{definition}[$\Gamma$-Support and Confusion Set] \label{def confuse}Fix a scalar $\Gamma>0$ and two vectors $\ab,\bb\in\R^p$. Define $\Gamma$-support of $\ab$ as $\supg{\ab}=\{i\bgl |a_i|\geq \Gamma,~1\leq i\leq p\}$. As a function of $\Gamma$, let us call features larger than $3\Gamma/2$ {\em{important}} and less than $\Gamma/2$ {\em{not important}}. $\Gamma$ confusion set between $\ab$ and $\bb$ is denoted by $\conf{\ab,\bb}$ and is defined as 
%\begin{align}
%\conf{\ab,\bb}=(\supt{\ab}-\suph{\bb})\bigcup(\supt{\bb}-\suph{\ab})\nn.
%\end{align}
%\end{definition}\vspace{-5pt}
%In words, the confusion set is the union of all the features that are important in one of the vectors and are not important in the other. Our next theorem shows the robustness of the weights learned by early-stopped gradient descent when labels are aligned with the principal eigendirections of $\X$. \vspace{-3pt}%For simplicity of notation we will assume $n\leq p$ which is the more interesting regime.
%%Given $\ab\in\R^n$, let $\ab_+\in\R^d$ denote its first $d$ entries and $\ab_-\in\R^{n-d}$ denote the remainder. 
%%Also given a matrix $\Ub$ denote its range space by $\Rc(\Ub)$.
%\begin{theorem}[Feature Robustness with Early-stopping]\label{early stop cor} Let the matrix $\X$ be as in Definition \ref{def cov} and fix $d,R$ and $r=r(d,R)$. Suppose for some parameter $\bt_\st\in\text{range}(\Vb_{1:d})$ and noise vector $\z$, the labels $\y$ obey 
%\[
%\y=\bar{\y}+\z\quad\text{where}\quad\bar{\y}=\X\bt_\st.
%\]
%Set $\z'=\Ub^T\z$ and coherence $\mu=\mu(\Vb_{1:r})$. Set learning rate $\eta\leq 1/\la_1$, initial point $\bt_0=0$ and run gradient iterations \eqref{GD} for $T={T_0}/(\eta\la_d)$ steps. The following bounds hold.
%
%\noindent$\bullet$ {\bf{Adversarial $\z$:}} For all $\Gamma\geq 2\mu(\e^{-T_0}\tn{\bt_\st}+\frac{\tn{\z'_{1:r}}}{\sqrt{\la_r}})$,% we have that 
%\begin{align}
%|\conf{\bt_\st,\bt_T}|\leq \frac{4T_0^2\tn{\z'_{r+1:p}}^2}{\Gamma^2R\la_d}.\label{adv bound}
%\end{align}
%\noindent$\bullet$ {\bf{Random $\z$:}} Suppose $\tsub{\z}\leq \sigma$. Let $\|\cdot\|_{2,\infty}$ return the largest $\ell_2$ norm among the rows of a matrix. For sufficiently large constant $C>0$, selecting
%\[
%\Gamma\geq C\sigma\sqrt{\log p} (\frac{T_0}{\sqrt{R\la_d}}+\frac{\|\Vb_{1:r}\|_{2,\infty}}{\sqrt{\la_r}})+2\mu \e^{-T_0}\tn{\bt_\st},%>2\tin{\bt_\st-\bt_T}.
%\]
%with probability at least $1-p^{-100}$, $|\conf{\bt_\st,\bt_T}|=0$.
%%\end{itemize}
%\end{theorem}
%{In words, Theorem \ref{early stop cor} establishes the entry-wise robustness of the model weights. Specifically, it determines threshold $\Gamma$ such that weights of the ground-truth function $\bt_\st$ that are larger than the threshold (which corresponds to prominent features) are identifiable. Adversarial bound \eqref{adv bound} bounds the number of confused features (per Def.~\ref{def confuse}) in terms of $\tn{\z'_{r+1:p}}$ which represents the projection of the noise on the tail of the eigenspectrum.} We remark that the role of the eigenspectrum and early-stopping in generalization and optimization is a well-studied topic \cite{yao2007early} however our focus is on the feature selection aspect. To further interpret Thm.~\ref{early stop cor}, let us consider a perfectly sparse setup with simplified assumptions on the eigenspectrum and incoherence.
%\begin{lemma}\label{simple lem} Let $C>0$ be an arbitrary constant. Let $\bt_\st$ be an $s$-sparse vector obeying $\tn{\bt_\st}\leq p^{C}$ and\\%\vspace{-5pt}
%$\bullet$ \text{Nonzeros are at least $1$:}~$\min_{\bt_{\star,i}\neq 0}|\bt_{\star,i}|\geq 1$,\\
%$\bullet$ \text{Nonzeros are not spiky:}~$\tin{\bt_\st}/\tn{\bt_\st}\leq C/\sqrt{s}$.
% %the absolute values of its nonzero entries are at least $1$, $\tin{\bt_\st}/\tn{\bt_\st}\leq C/\sqrt{s}$ and $\tn{\bt_\st}\leq p^{C}$. 
%
%${\cal{S}}_{\text{rnd}}$ be a $(d-1)$-dimensional uniformly random subspace in $\R^p$. Consider a design matrix $\X$ (as in Def.~\ref{def cov}) as follows. %\vspace{-8pt}
%%\begin{itemize} \vspace{-5pt}
%$\bullet$ {\bf{Spectrum:}} $\la_d\geq R\la_{d+1}$ and $1=\la_1\leq C\la_d$.\\%\vspace{-4pt}% and $\la_{d+1}\leq C\la_n$.
%$\bullet$ {\bf{Coherence:}} $\text{range}(\Vb_{1:d})=\text{span}(\{\bt_\st\}\cup {\cal{S}}_{\text{rnd}})$.
%%\end{itemize}  \vspace{-4pt}
%
%Suppose $\y=\X\bt_\st+\z$ where the noise level is $\sigma=\tsub{\z}$. There exists absolute constants $c,c_0>0$ such that if
%\[
%c_0\sigma^2\leq \frac{R}{\log^3p}\wedge \frac{p/d}{\log^2p}\wedge \frac{s}{\log p}.%\wedge \frac{p}{ds\log^2p}.
%\]
%Then, after $T_0=C\log p+2$ (normalized) gradient iterations as in Theorem \ref{early stop cor}, with probability at least $1-cp^{-3}\log p-d\e^{-p/8}$, hard thresholding the entries of $\bt_T$ at ${1}/{2}$ reveals the true sign/sparsity pattern of $\bt_\st$.
%\end{lemma}
%This lemma highlights the individual roles of $R$ (spikiness of the eigenspectrum), $s$ (sparsity level) and $d$ (the dimension of the relevant subspace) for accurate feature selection. $p/d\wedge s$ term arises due to the coherence of the $\text{range}(\Vb_{1:d})$ and $R$ term captures the weakness of the spectrum tail.




%Ignoring logarithmic terms, this lemma shows that tolerable noise amount for feature selection grows with spikiness of the spectrum $R$, sparsity level $s$ and the dimension of the label function subspace $d$.
%The following lemma is a simple application 
%\begin{theorem}
%\end{theorem}
%Then, we find
%\[
%\tin{\Vb_{r+1:p}\Db_-\z'_{r+1:p}}\leq \mu(\Vb_{r+1:p},\Db_-\z'_{r+1:p})\tn{\Db_-\z'_{r+1:p}}\leq \frac{T_0}{\la_d}\mu(\Vb_{r+1:p},\Db_-\z'_{r+1:p})\tn{\z'_{r+1:p}}.
%\]
%\begin{lemma} [$\ell_\infty$ bound for random noise] Let $\z\in\R^n$ be a zero-mean vector with subgaussian norm bounded by $\sigma$ and $\M\in\R^{n\times p}$ be a matrix. We have that
%\[
%\tin{\M\z}\leq.
%\]
%\end{lemma}
%\subsection{Further refinement via incoherence.}


==> experiments.tex <==
\section{Experiments}
In the experiment part, let us first discuss the setup for all experiments.

==> linear.tex <==

\vs\vs
\section{Importance and Covariance Bias for Linear Models}\label{sec linear}\vs\vs
% in connection to the importance Definition~\ref{def: weight impo}
%We first show that linear models have implicit bias in the form of covariance structure.   


%\vspace{-5pt}
%\subsection{Covariance structure}

%{\bf{Covariance structure:}} 
%For linear models, importance of a weight essentially captures the contribution of the corresponding feature. Thus, intuitively it should be invariant to how the features are scaled. However as we will discuss next, this is not necessarily the case when the problem is over-parameterized, which will reveal the role of implicit bias in terms of covariance structure. To formalize this, 
%Given the dataset $\Sc$ and $\Sc_{\La}$, w


% as well as kernel regression \cite{}
This section provides our results on pruning linear models and the role of feature covariance. Given a data distribution $\Dc$, we obtain a dataset $\Sc$ containing $n$ i.i.d.~samples $\Sc=(\x_i,y_i)_{i=1}^n\distas \Dc$. Let $(\x,y)\sim\Dc$ be a generic sample. We assume $(\x,y) \in (\R^p, \R)$ has finite second moments. 

\noindent {\bf{Covariance/Hessian structure:}} To understand the role of feature covariance (i.e.~Hessian) on pruning, we introduce a class of datasets where the input features are shaped by an invertible diagonal scaling matrix $\La\in\R^{p\times p}$ while output label $y$ is preserved. Here, a key motivation is modeling the properties of neural networks where the Hessian spectrum is not flat and often low-rank \cite{hastie2019surprises,sagun2017empirical,papyan2018full,mei2019generalization,arora2019fine}. The intuition is that the importance of a weight captures the contribution of the corresponding input feature and should be invariant to how the feature is scaled. Perhaps surprisingly, we will also show this intuition fails for over-parameterized problems. To proceed, given $\La$, we consider a distribution $\Dc_{\La}$, with samples $(\x^{\La},y)\sim\Dc_{\La}$ distributed as $(\La\x,y)$. Similarly, given $\Sc$, we generate a dataset $\Sc_{\La}=(\x^\La_i,y_i)_{i=1}^n$ where $\x^\La_i=\La\x_i$. We gather the data in matrix notation via \som{Consider better motivation}\som{In neural networks and kernels, design matrix may not be normalized which motivates an understanding of the impact of covariance structure, we will consider a class of problems}
\[
\X_\La=[\x^\La_1~\x^\La_2~\dots~\x^\La_n]^T\in\R^{n\times p} \quad \text{and}\quad \y=[y_1~y_2~\dots~y_n]^T \in \R^n.
\] 
%Also we define the dataset $\Sc_{\La}=(\x^\La_i,y_i)$ where $\x^\La_i=\La\x_i$. 
%Observe that the design matrix $\X_\La$ helps quantifying the impact of covariance structure on pruning.
%population The next lemma formalizes scaling invariance.
%where $\x \in \R^d$ and $y \in \R$. Given a prediction function $f$ parameterized by a vector $\bteta \in \R^p$ and a loss function $\ell(\cdot):\R\rightarrow\R$, we will investigate the properties of the Empirical Risk Minimization (ERM) problem
%Let $\{\X,\y\}\in\R^{n\times d}\times \R^n$ denote our dataset of size $n$ and $\bt\in\R^p$ denotes our model.  For notational simplicity, throughout, we assume $n\leq p$ which is the more interesting setup for feature selection and deep learning problems. Then, given a prediction function $f$, one can solve a Empirical Risk Minimization (ERM) problem
To proceed, using quadratic loss, we define the empirical (training) and population (test) losses,% as follows,
\begin{align}
\Lch_{\La}(\bt):=\frac{1}{n}\sum_{i=1}^n (y_i-\bt^T\x^{\La}_i)^2=\frac{1}{n}\tn{\y-\X_\La\bt}^2\quad\text{and}\quad\Lc_{\La}(\bt):=\E[(y-\bt^T\x^{\La})^2].\label{eqn: ERM linear}
\end{align}
Let $\bth^{\La}, \btb^{\La}$ be the global minima of $\Lch_{\La}$ and $\Lc_{\La}$ respectively. Let $\bSi=\E[\x\x^T]$ be the population covariance and $\bb=\E[\x y]$ be the cross-correlation. For simplicity, we assume $\bSi$ is full-rank. {\em{We will drop the subscript $\La$ when $\La=\Iden_p$}}. The solutions $\bth^{\La}, \btb^{\La}$ are given by 
\[
\bth^{\La}=\X^\dagger_{\La} \y\quad\text{and}\quad\btb^{\La}=\La^{-1}\bSi^{-1}\bb,
\] 
respectively, where $\dagger$ denotes the pseudo-inverse. The following lemma is instructive in understanding the weight importance and invariance to feature scaling for the least-squares problem above~\eqref{eqn: ERM linear}.%\som{Should we require $\bSi$ to be invertible}
%discusses the proposed measurement of weight importance on linear quadratic models and neural networks. Firstly, let us define the weights importance on linear model and quadratic loss as following.
\vs\begin{lemma}[Pruning with Population]\label{cov importance}
	%Given matrix $\X\in\R^{n\times d}$ where each line is an input sample and the ground truth parameter $\bt_{oracle}\in\R^d$. Let $\Sigma=\X^\top\X$ denotes the covariance of $X$ and $\y=\X\bt_{oracle}+\sigma$ where $\sigma$ is random gaussian noise. For minimizing quadratic loss $\bth=\arg \min_{\bth}1/2{\tn{\y-\X\bth}^2}$, the weight importance for i-th entry of $\bth$ is defined as
	%\begin{align}
	%	\Im_{\bth_i}=\abs{\sqrt{\diag{(\Sigma)}}_i\bth_i}
	%\end{align}
	%Define the covariance matrix $\bSi=\E[\x\x^T]$ and the cross-correlation $\bb=\E[\x y]$.
	Let $\btb^{\La}$ be the minimizer of population loss and fix $\ix \subseteq [p]$. NI $\Icn_\ix(\btb^\La)$ and HI $\Ic^H_\ix(\btb^\La)$ w.r.t.~population loss $\Lc_\La$ are invariant under invertible diagonal $\La$. If the covariance $\bSi$ is also diagonal, then NI and HI are equal. In contrast, MI is $\La$ dependent via $\Ic^M_\ix(\btb^\La)=\sum_{i\in \ix}\La_{i,i}^{-2}{\btb_i}^2$ where $\btb=\btb^{\Iden_p}$ is the original model.
	
%	For any diagonal $\La$ and any , NI and HI satisfies\som{Need general covariance version. Should be matrix inversion lemma or similar to Lemma C.1}% Given the loss function~\eqref{eqn: ERM linear}, let $\bSi = \frac{1}{n}\X^T\X$ be the empirical covariance matrix. Then, the weight importance of $i$-th element of $\bt$ is given by
%	\begin{align}
%	\Icn_\ix(\btb^\La) = \Ic_\ix^H(\btb^\La)=\sum_{i\in \ix}\bSi_{i,i}{\btb_i}^2.
%	\end{align}
%	Additionally, 
	%\[
	%\Ic^M_\ix(\btb^\La)=\sum_{i\in \ix}\La_{i,i}^{-2}\bSi_{i,i}{\btb_i}^2.
	%\]
\end{lemma}
%\som{Add discussion on magnitude shining when identity cov}
This lemma states that NI and HI are invariant to scaling and coincide when features are uncorrelated. On the other hand, MI suffers from feature scaling. As the features get larger, the corresponding weight decreases which results in an artificial decrease in importance. This highlights a fundamental shortcoming of MP and necessity of feature normalization, which was previously discussed in the literature~\cite{santurkar2018does,ioffe2015batch,jayalakshmi2011statistical,ekenel2006norm}. In Sections \ref{train loss} and \ref{neural sec}, we will see that MP fails as soon as the problem is not well-conditioned either in terms of covariance spectrum or neural network initialization.
%\som{Find some reference mentioning this. Has to be known!!!}

%which include the test loss (which has access to infinite samples)
Invariance to feature scaling is a property of over-determined problems ($n>p$) which admit unique solution (population loss is a special case with $n=\infty$). Focusing on training loss, suppose $\X\in\R^{n\times p}$ is not rank deficient. Then, the minimum-norm solution $\bth^\La$ has the form
\begin{align}
\bth^\La=\begin{cases}\La^{-1}\bth,\quad\text{when}\quad n\geq p,\\
\La\X^T(\X\La^2\X^T)^{-1}\y,\quad\text{otherwise.}\end{cases}\label{LS soln}
\end{align}
When $n\geq p$, we trivially have $(\bth^{\La})^T\x^\La=\bth^T\x$, thus $\bth$ and $\bth^\La$ achieve the exact same test/training loss. On the other hand, for over-parameterized problems ($n<p$), which is the regime of interest for  neural network pruning, this is no longer the case, and we will see that $\La$ plays a critical role in the eventual test performance as it dictates which solution the optimization problem selects.
% as well as compressed sensing

%for linear models the importance is captured by covariance scaling. This implies that when the input data has a covariance then the magnitude-based pruning results in reduced test accuracy as compared to weight-importance pruning. 

%\subsection{Training Loss, Over-parameterization, and Implicit Bias} 
\vs\subsection{Characterizing Pruning Performance and Covariance Bias}\label{train loss}\vs
% by characterizing their performances in a high-dimensional setup. Our analysis reveals the importance of implicit bias in the form of covariance structure, in pruning performance. 
\mc{repeat $y=\x^\top\bt+z$ on line 175 and 176}
In this section, we provide analytical formulas which enable us to compare different pruning methods and assess implicit covariance bias when $n<p$ under a realizable dataset model. Suppose $(\x_i)_{i=1}^n\distas\Nn(0,\Iden_p)$ so that $\bSi=\Iden_p$ and $\bSi_\La:=\E[\x^\La(\x^\La)^T]=\La^2$. Given a ground-truth vector $\btb\in\R^p$ (which corresponds to the population minima), we generate the labels via $y=\x^T\btb+z$ and\vs
\[
y_i=\x_i^T\btb+z_i\quad\text{for}\quad 1\leq i\leq n,
\]
%\som{Refine this discussion}
%$\bth^\La$ given via 
where $z,(z_i)_{i=1}^n\distas\Nn(0,\sigma^2)$ are the additive noise. We will study the minimum norm least-squares solution \eqref{LS soln} which is also the solution gradient descent converges when initialized from zero. To assess pruning performance, we need to quantify the test loss of the pruned solution $\Pi_{s}(\bth)$. 

\vs
\noindent{\bf{Connection to denoising:}} We accomplish this by {\em{relating the test loss of the pruned model to the risk of a simple denoising problem}}. In essence, this denoising question is as follows: Given noisy measurements $\bt_{\text{nsy}}=\btb+\g$ of a ground-truth vector $\btb$ with $\g\sim\Nn(0,\sigma^2\Iden_p)$, what is the pruning error $\E[\tn{\Pi_s(\bt_{\text{nsy}})-\btb}^2]$? Note that this error typically doesn't have a closed form answer as hard-thresholding is not a continuous function, however, it greatly simplifies the original problem of solving least-squares. We also note that if one uses soft-thresholding (i.e.~shrinkage) operator for pruning, closed form solution is available. The fundamental connection between denoising and linear inverse problems are studied for under-parameterized least-squares and lasso regression \cite{donoho2013accurate,donoho2009message}. Our connection to denoising is established by connecting the distribution of the $\bth^\La$ to an auxiliary distribution described below.
\mc{ Line 186, "inverse problems are studied", are-> is}
%Observe that pruning even under a simple denoising setup doesn't have a closed form solution. Namely, given noisy measurements $\bth=\btb+\g$ with $\g\sim\Nn(0,\sigma^2\Iden_p)$, what is the pruning error $\E[\tn{\Pi^M_s(\bth)-\btb}^2]$? There is no clean Noise $\g$ can change the set of pruned weights discontinuously.

% as a result there is no closed form formula for $\text{err}_s$.

%hard-thresholding is not a nice Lipschitz function and 
%\text{err}_s=
%\cite{donoho1995noising}

%Observe that, the pruning functions ($\Pi^N_{s}, \Pi^M_{s},\Pi^H_{s}$) are not Lipschitz thus a closed-form solution for exact test performance analysis is unlikely. 

% circumvent this issue by directly capturing the asymptotic distribution of the over-parameterized solution to the least-squares problem~\eqref{eqn: ERM linear} via 

% Note that there are infinitely many minimizers of empirical risk however 
% loss however \eqref{}Clerly,  finite-sample least-squares problem \eqref{eqn: ERM linear} by minimizing $\Lch_\La$ and pruning the optimal solution.


%Note that, the test loss of $\bth^\La$ follows
%\[
%\Lc(\bt)=\tn{\La\bth^\La-\btb}^2+\sigma^2.
%\]

%Note that, $\bth$ is a noisy version of the ground-truth parameter $\btb$ and pruning is particularly difficult to analyze as it is not even a Lipschitz function and even if one knows the true distribution of $\bth$, a closed form solution is not expected as the order of the relative importance of the weights might randomly change. We instead provide formulas that can predict
 %we will consider a high-dimensional setup 

%\som{add further discussion on 3.2} 
\vs\vs
\begin{definition}[Auxiliary distribution] \label{aux_def}Fix $p>n\geq 1$ and set $\kappa=p/n>1$. Given $\sigma>0$, positive definite diagonal matrix $\La$ and ground-truth vector $\btb$, define the unique non-negative terms $\Xi,\Gamma,\bz\in\R^p$ and $\bg\in\R^p$ as follows\vspace{-12pt}
\begin{align}
&\Xi>0\quad\text{is the unique solution of}\quad 1=\frac{\kappa}{p}\sum_{i=1}^p\frac{1}{1+(\Xi\La_{i,i}^2)^{-1}},\label{aux solve}\\
&\Gamma=\frac{\sigma^2+\sum_{i=1}^p\bz_i^2\btb_i^2}{\kappa(1-\frac{\kappa}{p}\sum_{i=1}^p{(1+(\Xi\La_{i,i}^2)^{-1})^{-2}})},\nn\\
&\bz_i=\frac{1}{1+\Xi\La_{i,i}^2}\quad\text{and}\quad \bg_i=\frac{\kappa\sqrt{\Gamma}}{1+(\Xi\La_{i,i}^2)^{-1}}\quad\text{for}\quad 1\leq i\leq p.\nn
\end{align}
Let $\h\sim\Nn(0,\frac{1}{p}\Iden_p)$. Define the auxiliary vector $\bta^\La$ of the ground-truth $\btb$ as% of $\hat{\bt}$ can be approximated as
\begin{align}
\bta^\La= \La^{-1}[(\onebb_p-\bz)\odot\btb+\bg\odot\h].\label{aux dist def}
\end{align}
\end{definition}
We remark that this definition can be adapted to asymptotic setup $p\rightarrow\infty$ assuming covariance spectrum converges (e.g.~discrete sum over entries converges to an integral). In the special case of identity covariance ($\bSi=\Iden_p$), $\bta$ reduces to $\bta=\frac{1}{\kappa}\btb+\sqrt{\frac{\sigma^2}{\kappa-1}+\frac{(\kappa-1)\tn{\btb}^2}{\kappa^2}}\h$. This distribution arises from applying Convex Gaussian Min-Max Theorem (CGMT) \cite{Gor,Gor2,thrampoulidis2015regularized,OymLAS,thrampoulidis2018precise} to over-parameterized least-squares. CGMT provides a framework for predicting the asymptotic properties of optimization problems involving random matrices by connecting them to simpler auxiliary optimizations involving random vectors. Thus, based on CGMT, $\bth^\La$ and the auxiliary vector $\bta^\La$ are expected to have similar distributional properties and $\bta^\La$ can be used as a proxy to capture the properties of $\bth^\La$. In supplementary, we discuss to what extent this distributional similarity can be formalized (e.g.~for Lipschitz functions). Note that, after solving for $\bz,\bg$ in \eqref{aux solve}, we can sample from the auxiliary distribution which is a noisy version of $\btb$ which connects us to denoising. To proceed, our analytic formulas for the test error of an $s$-sparse model via MP and HP takes the following form:
\begin{align}
\text{MP loss:}~\E_{\h}[\tn{\La\Pi^M_s(\bta^\La)-\btb}^2]+\sigma^2,\quad \text{HP loss:}~\E_{\h}[\tn{\Pi^M_s(\La\bta^\La)-\btb}^2]+\sigma^2.\nn%\label{prune loss}
\end{align}
%we will show that the test loss of the pruned auxiliary vector, which is simply $\E_{\h}[\tn{\La\Pi^N_{\ix}(\bta^\La)-\btb}^2]+\sigma^2$ successfully predicts that of pruned empirical risk minimizer $\bth$.


%simply addsis simply a diagonal multiplication and  whereas solving for $\bth$ requires a pseudo-inverse.
% under over-parameterization
%$\bSi=\Iden_p$, 

Next, we verify our performance prediction and study the role of covariance structure $\La$. We generate $\btb$ with polynomially decaying entries, specifically $\btb_i=1/(1+4i/p)^2$, and then scale it to unit Euclidian norm. Recall that original covariance is identity, thus initial larger entries of $\btb$ are more important for population risk. In our experiments, we parameterize $\La$ by a scalar $\la$ and set it as %\ysatt{what $n,p$ and $\sigma$ are used to generate figure 1}
%\ysatt{sub-captions are redundant}
%$\La:=\La^\la$
\begin{align}
\La_{i,i}=\begin{cases}\la\quad\text{if}\quad 1\leq i\leq p/10,\\1\quad\text{if}\quad i>p/10.\end{cases}\label{linear scaling}
\end{align}
This choice modifies the most important 10\% weights of the problem. We consider $\la\in \{1/2,1,5\}$. As formalized in Thm.~\ref{lem win}, when $\la>1$, we expect a positive covariance bias since important weights are aligned with the principal directions of the covariance and are easier to learn. In Figures \ref{fig:positive} and \ref{fig:negative}, the lines are the analytical predictions based on Definition \ref{aux_def} and the markers are performance of the actual least-squares solution which nicely match for all pruning methods and $\la$. Figure \ref{fig:positive} contrasts $\la=1$ and $\la=5$. For $\la=1$, MP and HP coincide as the Hessian is identity. However when $\la=5$, HP performs much better than $\la=1$ for all sparsity levels. MP drastically fails for small sparsity levels as the initial weights of $\bth^\La$ are important but small due to the $\la$-scaling thus MP inaccurately ignores them. Decreasing magnitudes with increasing $\la$ is more clear for under-parameterized case (via \eqref{LS soln}) however $\La^{-1}$ dependence is also visible in \eqref{aux dist def}. Fig \ref{fig:negative} additionally highlights $\la=1/2$ which reduces the covariance and scales up the coefficients of the important weights. This leads to a negative bias because covariance structure guides the solution away from important weights. While both MP and HP performs worse than $\la=1$ case, HP performs worse due to additional penalization of the initial important weights. Finally, covariance bias is visualized in Figure \ref{fig:covariance} which displays the test NI (for $\btb$) and the training NI's (for $\bth^\La$) of the first $s$ weights. When $\la=5$, initial weights, which are important for test, have a larger training NI. As $\la$ gets smaller, remaining weights, which are not as important for test, have larger say during training and pruning performance degrades. Our Theorem \ref{lem win} formalizes these by quantifying the contributions of different weights during training.%training dynamics.
\mc{I made the label of fig 1 a bit smaller}
%covariance weighting.
%Appendix A in the supplementary provides further theoretical justification for this statement. 
% and the corresponding spectrum is visualized in Figure \ref{fig:covariance}
%	\begin{subfigure}{1.8in}
%	\begin{tikzpicture}
%	\node at (0,0) {\includegraphics[scale=0.22]{figs/covariance_lambda}};
%	\node at (-2.35,0) [rotate=90,scale=1.]{Covariance};
%	\node at (0,-1.8) [scale=1.]{Weight Index};
%	\end{tikzpicture}\vspace{-3pt}\caption{$\la=1$ corresponds to $\bSi=\Iden_p$ and results in same pruning performance. 
%	}\label{fig:covariance}\vspace{-0.2cm}
%	\end{subfigure}
	
\begin{figure}[t!]
	\centering
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{figs/positive_bias}};
	\node at (-2.35,0) [rotate=90,scale=.8]{Test loss};
	\node at (0,-1.8) [scale=.8]{Fraction of non-zero ($s/p$)};%Each bar in the figure shows the correlations' geometric mean of datasets in this group when training to corresponding non-zero level. 
	\end{tikzpicture}\vspace{-3pt}\caption{%$\la=1$ corresponds to $\bSi=\Iden_p$. 
	\small{Pruning with $\la\in\{1,5\}$}}\label{fig:positive}\vspace{-0.2cm}
	\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{figs/negative_bias}};
	\node at (-2.35,0) [rotate=90,scale=.8]{Test loss};
	\node at (0,-1.8) [scale=.8]{Fraction of non-zero ($s/p$)};%Each bar in the figure shows the correlations' geometric mean of datasets in this group when training to corresponding non-zero level. 
	\end{tikzpicture}\vspace{-3pt}\caption{%$\la=1$ corresponds to $\bSi=\Iden_p$. 
	\small{Pruning with $\la\in\{1,1/2\}$}}\label{fig:negative}\vspace{-0.1cm}
		\end{subfigure}
	\begin{subfigure}{1.8in}
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.22]{figs/natural_importance}};
	\node at (-2.35,0) [rotate=90,scale=.8]{Natural Importance};
	\node at (0,-1.8) [scale=.8]{First $s/p$ entries};
	\end{tikzpicture}\vspace{-3pt}\caption{\small{NI of the first $s$ entries}}
	\label{fig:covariance}\vspace{-0.2cm}
	\end{subfigure}
		\caption{\small{In (a) and (b), the lines are the analytical prediction from Def~\ref{aux_def} and markers are the actual min-norm solution. $p=1000, \kappa=p/n = 5/3$ and $\sigma = 0.1$. (c) Natural importance associated with the first $s$ weights. For $\la=5$, (a) HP achieves better performance and (c) training and test NI have a better match.}}\vspace{-15pt}
\end{figure}
%\som{Make a bigger deal out of this}
%Observe that, thisto be a diagonal matrix where first $p/10$ entries are equal to $\la$. Specifically  In Figure \ref{} and \ref{}, We by $\la$ by 
%\begin{definition}[Auxiliary distribution] Set $\pbar=p/n$ and $\sbar=s/n$. Then, define the quantities
%\begin{align}
%&\Lambda\quad\text{is solution of}\quad n=\sum_{i=1}^p\frac{1}{1+(\Lambda\la_i)^{-1}},\\
%&\zeta_i=\frac{1}{1+\Lambda \la_i},\\
%&\gamma_i=\frac{c}{n(1+(\Lambda \la_i)^{-1})}\quad\text{where}\quad n(\sigma^2+\sum_{i=1}^n \gamma_i^2+\la_i\zeta_i^2\bt_i^2)=\Gamma^2.
%\end{align}
%Define the auxiliary distribution $\bt_{aux}$ as% of $\hat{\bt}$ can be approximated as
%\[
%\bta\sim (1-\zeta)\odot\bt-\bSi^{-1/2}\gamma\odot\g.
%\]
%\end{definition}

%Fig~\ref{fig:linear_theory} shows the comparison of MP and HP as well as covariance choices with scalings $\la=1$ and $\la=5$ by plotting the test loss of $\Pi^M_s(\bth^\La),\Pi^H_s(\bth^\La)$. various pruning methods with the importance-based pruning. The dash lines show the pruning result on $i.i.d.$ samples where the magnitude and importance-based pruning performs similar because of the absence of feature covariance. The solid lines shows that importance-based pruning significantly outperforms the magnitude pruning which leads to the key claim that implicit bias of datasets guides the training process and pruning criterion. Furthermore, Fig~\ref{fig:linear_pruning} provides the motivation to look into the Jacobian/Hessian-based pruning in complicated nonlinear models such as neural networks.
%Then, the test errors are given by
%\begin{align}
%&\Lc(\bth)=\sigma^2+\sum_{i=1}^p\gamma_i^2+\la_i\zeta_i^2\bt_i^2\\
%&\Lc(\tbh)=\sigma^2+\sum_{i=1}^s(\gamma_i^2+\la_i\zeta_i^2\bt_i^2)+\sum_{i=s+1}^p\la_i\bt_i^2.
%\end{align}
%\begin{lemma}[Invariance to Scaling] Fix scaling matrix $\La\in\R^{p\times p}$. Consider a distribution $\Dc_{\La}$ where $(\x_{\La},y)$ is distributed as $(\La\x,y)$ where $(\x,y)\sim \Dc$. We have that
%\[
%\]
%\end{lemma}
%Clearly, magnitude-based pruning and Hessian-based pruning coincides when covariance is identity. \dots



%\section{Exploring Pruning Mechanics for Neural Nets}\label{neural sec}
%%For the neural network, recent literature \cite{jacot2018neural,su2019learning,du2019gradient,chizat2019lazy,oymak2019towards,zou2018stochastic} indicate that Jacobian feature map $\Jb(\bt)=\frac{\pa f(\bt)}{\pa \bt}\in\R^{n\times p}$ acts as an ``instantaneous'' design matrix and governs the optimization dynamics via the first order approximation
%%\begin{align}
%%f(\bt+\Delta)\approx f(\bt)+\Jb(\bt)\Delta.\label{nn jacob}
%%\end{align}
%%This approximation is also at the core of the recent works on Neural Tangent Kernel \cite{jacot2018neural,du2018gradient}. Hence, properties of $\Jb$ may dictate which weights have a stronger say in the network's decision than others. Motivated by Def.~\ref{cov importance}, we define weight importance on neural network based on the Jacobian feature map as following.
%%
%%\begin{definition}[Weight importance on neural network]\label{jac importance}
%%Given dataset $(\X,\y)\in\R^{n\times d}\times\R^n$ and neural network $f$ parameterized by $\bt\in\R^p$. Let $\Jb(\bt)=\frac{\pa f(\bt)}{\pa \bt}\in\R^{n\times p}$ which is the derivative of network output w.r.t. parameters. The weight importance for i-th entry of $\bt$ is defined as
%%	\begin{align}
%%	\Im_{\bt_i}=\abs{\sqrt{\diag{(\Jb^\top\Jb)}}_i\bt_i}
%%	\end{align}
%%\end{definition}
%
%Hence, In Fig.~\ref{fig:compare_purining_C10_1}, we train a simple 2-layer neural network $f(\X)=\V\phi(\W\X^\top)$ on MNIST where $\W\in\R^{129\times784}$ and $\V\in\R^{10\times129}$ and we initialize the $\W_0$ and $\V_0$ using \textit{He normal}\cite{he2015delving}. In order to change the scaling of layers' initialization but preserve the initial output range, we use the factor $\lambda$ to scale the std of $\W$ to $\text{std}(\W_0)\lambda$ and $\V$ to $\text{std}(\V_0)/\lambda$ where $\text{std}(\M)$ denotes the standard derivation of all entries of matrix $\M$ . In Fig.~\ref{fig:compare_purining_C10_1}, the magnitude pruning failed with larger or smaller $\lambda$ because of the magnitude imbalance between layers. But hessian-based pruning in Fig.~\ref{fig:compare_purining_C10_2}
%
%\mli{todo: discuss the smaller weight larger importance using another figure (the mean/std of each layer's weights and jacobian)}
%
%Furthermore, the covariance and jacobian based pruning are tightly relevant to hessian based pruning when the model reaches global minima. \mli{todo: discussion}
%
%\mli{importance: how much removing entries changes test loss-> linear iid data/ covariance data/ covariance->jacobian,NTK papers->hissian -> ablation idea, set to zero, to understanding training, set to initial (for Thm 3.2). https://dl.acm.org/doi/pdf/10.5555/3305381.3305576?download=true.  In practice, weight pruning works well, jacobian pruning doesn't amazing better. because initialization is good. }
%
%\begin{figure}[t!]
%	\centering
%	\begin{subfigure}{1.8in}
%	\begin{tikzpicture}
%	\node at (0,0) {\includegraphics[scale=0.22]{figs/covariance_lambda}};
%	\node at (-2.35,0) [rotate=90,scale=1.]{Covariance Spectrum};
%	\node at (0,-1.8) [scale=1.]{Fraction of non-zero};%Each bar in the figure shows the correlations' geometric mean of datasets in this group when training to corresponding non-zero level. 
%	\end{tikzpicture}\vspace{-3pt}\caption{$\la=1$ corresponds to $\bSi=\Iden_p$. $\la=5$ results in positive implicit bias for Hessian pruning.}\label{fig:covariance}\vspace{-0.2cm}
%	\end{subfigure}
%	\begin{subfigure}{1.8in}
%	\begin{tikzpicture}
%	\node at (0,0) {\includegraphics[scale=0.22]{figs/positive_bias}};
%	\node at (-2.35,0) [rotate=90,scale=1.]{Test loss};
%	\node at (0,-1.8) [scale=1.]{Fraction of non-zero};%Each bar in the figure shows the correlations' geometric mean of datasets in this group when training to corresponding non-zero level. 
%	\end{tikzpicture}\vspace{-3pt}\caption{$\la=1$ corresponds to $\bSi=\Iden_p$. $\la=5$ results in positive implicit bias for Hessian pruning.}\label{fig:positive}\vspace{-0.2cm}
%	\end{subfigure}
%	\begin{subfigure}{1.8in}
%	\begin{tikzpicture}
%	\node at (0,0) {\includegraphics[scale=0.22]{figs/negative_bias}};
%	\node at (-2.35,0) [rotate=90,scale=1.]{Test loss};
%	\node at (0,-1.8) [scale=1.]{Fraction of non-zero};%Each bar in the figure shows the correlations' geometric mean of datasets in this group when training to corresponding non-zero level. 
%	\end{tikzpicture}\vspace{-3pt}\caption{$\la=1$ corresponds to $\bSi=\Iden_p$. $\la=1/2$ results in negative implicit bias for both prunings.}\label{fig:negative}\vspace{-0.2cm}
%		\end{subfigure}
%\end{figure}
%
%\begin{figure}[t!]
%	\centering
%	\begin{subfigure}{2.7in}
%		\begin{tikzpicture}
%		\node at (0,0) {\includegraphics[scale=0.45]{figs/Importance_layer_1}};
%		\node at (-3.5,0) [rotate=90,scale=.8]{Importance};
%		\node at (0,-2.3) [scale=.8]{$\lambda$};%Each bar in the figure shows the correlations' geometric mean of datasets in this group when training to corresponding non-zero level. 
%		\end{tikzpicture}\vspace{-3pt}\caption{First layer's importance on various measurements }\label{fig:Importance_layer_1}\vspace{-0.2cm}
%	\end{subfigure}\begin{subfigure}{2.7in}
%		\begin{tikzpicture}
%		\node at (0,0) {\includegraphics[scale=0.45]{figs/Importance_layer_2}};
%		\node at (-3.5,0) [rotate=90,scale=.8]{Importance};
%		\node at (0,-2.3) [scale=.8]{$\lambda$};%Each bar in the figure shows the correlations' geometric mean of datasets in this group when training to corresponding non-zero level. 
%		\end{tikzpicture}\vspace{-3pt}\caption{Second layer's importance on various measurements }\label{fig:Importance_layer_2}\vspace{-0.2cm}
%	\end{subfigure}
%\end{figure}
%
%\begin{figure}[t!]
%	\begin{subfigure}{2.7in}
%		\begin{tikzpicture}[scale=1,every node/.style={scale=1}]
%		\node at (0,0) {\includegraphics[scale=0.45]{figs/retrain_naive_acc.pdf}};
%		\node at (-3.5,0) [rotate=90,scale=.8]{Test accuracy};
%		\node at (0,-2.3) [scale=.8]{Fraction of non-zero};
%		%\node at (2.4,0) [rotate=90,scale=.8]{$\log_{10}{\lambda}$};
%		\end{tikzpicture}\caption{Test accuracy using naive weight magnitude pruning. }\label{fig:compare_purining_C10_1}
%	\end{subfigure}
%	\begin{subfigure}{2.7in}
%		\begin{tikzpicture}[scale=1,every node/.style={scale=1}]
%		\node at (0,0) {\includegraphics[scale=0.45]{figs/retrain_jacobian_acc.pdf}};
%		\node at (-3.5,0) [rotate=90,scale=.8]{Test accuracy};
%		\node at (0,-2.3) [scale=.8]{Fraction of non-zero};
%		%\node at (2.4,0) [rotate=90,scale=.8]{$\log_{10}{\lambda}$};
%		\end{tikzpicture}\caption{Test accuracy using Hessian-based pruning.}\label{fig:compare_purining_C10_2} 
%	\end{subfigure}
%	\caption{In Fig.~\ref{fig:compare_purining_C10}, we investigate two pruning methods on MNIST training on 2-layer fully connect neural network with different initialization under softmax activation and cross-entropy loss.  }\label{fig:compare_purining_C10} 
%\end{figure}
%
%
%
%
%% if the spectrum of the problem is aligned with prominent features, 
%%Secondly, we will  why feature selection is possible without explicit sparsity regularization. 
%
%%Indeed to obtain good solutions such explicit regularization is often crucial to have any chance of success. 


==> neuralnet.tex <==

\vs\vs\section{Hessian Bias and the Role of Initialization for Neural Nets}\label{neural sec}\vs\vs
%So far we discussed pruning and implicit bias in linear models. 
This section extends our discussion of importance and pruning to another fundamental model class: neural networks with one-hidden layer. Suppose input dimension is $d$, output dimension is $K$ and the network has $m$ hidden units. Such a network with ReLU activation is given by $f_{\bt}(\x)=\V\act{\W\x}$, where $\W\in\R^{m\times d}$ and $\V\in\R^{K\times m}$ are the input and output layers respectively and $\bt=(\W,\V)\in\R^{p=(d+K)m}$ is the vector composed of the entries of $\W,\V$. Let $\ixi$ and $\ixo$ denote the index of the entries of $\W,\V$ in $\bt$. Given a dataset $\Sc=(\x_i,y_i)_{i=1}^n$ and loss $\ell$, we minimize\vs\vs% the loss
\begin{align}
\Lc(\bt)=\frac{1}{n}\sum_{i=1}^n\ell(y_i,f_{\bt}(\x_i)).\label{loss}
\end{align}
{\bf{Equivalent networks:}} To study neural net pruning and initialization, we shall consider a class of networks $\bt^\la=(\la\W,\la^{-1}\V)$ generated from a base network $\bt^1=(\W,\V)$. Observe that all vectors $\bt^\la$ implement the same function due to the linearity of ReLU however magnitudes of layers are varying. The following lemma shows how the parameter $\la$ affects MI, HI, and Hessian.
%Throughout this section, we will focus on shallow neural networks of the form $f_{\bt}(\x)=\V\act{\W\x}$ where $\bt\in\R^{}$ is the vector composed of the entries of input layer $\W$ and output layer $\V$. \dots
\mc{MI,HI and partial derivatives obey --Line 236}

\begin{lemma} \label{simple hessian gradient}Consider the loss \eqref{loss} and class of networks $(\bt^\la)_{\la>0}$. For all $\la>0$, MI, HI and partial Hessians w.r.t.~input/output layer weights $\W,\V$ obey%\som{Consider removing MI which is trivial}
%[Importance -- Shallow Network] 
\begin{align}
&\Ic^M_\ixi(\bt^\la)=\la^2\Ic^M_\ixi(\bt^1)\quad\text{and}\quad\Ic^M_\ixo(\bt^\la)=\la^{-2}\Ic^M_\ixo(\bt^1),\nn\\
&\Ic^H_\ixi(\bt^\la)=\Ic^H_\ixi(\bt^1)\quad\text{and}\quad\Ic^H_\ixo(\bt^\la)=\Ic^H_\ixo(\bt^1),\label{constant HI}\\
&\frac{\pa^2}{\pa^2{\W}}\Lc(\bt^\la)=\la^{-2}\frac{\pa^2}{\pa^2{\W}}\Lc(\bt^1)\quad\text{and}\quad\frac{\pa^2}{\pa^2{\V}}\Lc(\bt^\la)=\la^2\frac{\pa^2}{\pa^2{\V}}\Lc(\bt^1).\label{gradient change}
\end{align}
\end{lemma}
In words, increasing $\la$ increases MI, preserves HI, and decreases the Hessian magnitude for the input layer and has the reverse effect on the output layer. Suppose we train the network from initializations $\bt^\la$ on \eqref{loss}. What happens at the end of the training as a function of $\la$? Does eventual MI and HI exhibit similar behavior to initialization? What about NI?


\mc{Don't know whether "interpolation to training data" is correct grammar or not --Line 244/245.}

% in training
To answer these, in Figure \ref{fig:Importance_layer}, we conduct an empirical study on MNIST by training a one-hidden layer network with cross-entropy loss. Here $m=1024$, $d=784$ and $K=10$. We set $\bt^{1}_{\ini}=(\W_\ini,\V_\ini)$ with \textit{He normal} initialization \cite{he2015delving}. We then train networks with $\la$-scaled initializations $\bt^\la_\ini=(\la\W_\ini,\la^{-1}\V_\ini)$. Let $\bt_\fn^{(\la)}=(\W_\fn^{(\la)},\V_\fn^{(\la)})$ be the final model obtained by training until interpolation to training data (or maximum 150 epochs). Figures~\ref{fig:Importance_layer_1} and \ref{fig:Importance_layer_2} display MI, HI, and NI for input and output layers respectively. Here, for NI, we use {\em{Init-Pruning}} and quantify importance of a layer (e.g.~$\W_\fn^{(\la)}$) with respect to its initial weights (e.g.~$\W_\ini^{\la}=\la\W_\ini$). Observe that, regular pruning is not informative as setting a layer to zero kills the network output.



%The orange line (HI) in Fig.~\ref{fig:Importance_layer_1},~\ref{fig:Importance_layer_2} are results of soft pruning where we replace $\W_\fn^\la$ to $\W_0^\la$ in Fig.~\ref{fig:Importance_layer_1} and $\V_\fn^\la$ to $\V_0^\la$ in Fig.~\ref{fig:Importance_layer_2}. 

% (i.e.~reference is initialization $\bt_0^\la$)
% rather than regular pruning


% To visualize the information in a similar range, we draw the green HI line with $10^5$ scaling.
\noindent{\bf{Understanding MI and HI:}}\mc{I changed legend's position and text for fig 2c. change w,v to input NI, output NI} Figures~\ref{fig:Importance_layer_1} and \ref{fig:Importance_layer_2} show that initial and final MI exhibit a near perfect match. The initial HI stays constant as predicted by Lemma~\ref{simple hessian gradient}. Final HI increases with $\la$ for both layers, however it can be verified that the ratio of HI between input and output layers is approximately preserved. Perhaps surprisingly, Lemma~\ref{simple hessian gradient} seems to predict not only the initial importance but also the MI/HI of the final network. Fortunately, this can be mostly explained by the optimization dynamics of wide and large networks where gradient descent finds a global optima close to initialization and {\em{final weights (and Hessian) do not deviate much from initial ones}} \cite{chizat2019lazy,du2018gradient,jacot2018neural,allen2019convergence}.\mc{\cite{lee2019wide} also about wide network and linearization -Line 256}

\mc{No more $10^5$HI, but "we draw the blue line as $\sqrt{MI}$ which is proportional to $\la$" --Line 249/250}



%\som{check this part!!!}%Moreover, 
\vs
In Figures~\ref{fig:compare_purining_C10_1} and \ref{fig:compare_purining_C10_2}, we first prune $\bt_\fn^{(\la)}$ to a fixed nonzero fraction and then retrain the pruned weights from the same initialization (i.e.~\cite{frankle2019lottery}). MP is only competitive with HP when $\la=1$ where input and output layer entries have similar magnitude due to He initialization. In Fig.~\ref{fig:compare_purining_C10_1}, as $\la$ grows output layer becomes small and gets fully pruned. As $\la$ gets smaller, eventually input layer is fully pruned. Here, what is rather remarkable is the robustness of HP for full range of $\la$ choices which arises from \eqref{constant HI}. Arguably, HI being invariant to $\la$ makes it more attractive than NI as it avoids the issue of {\em{layer death}} i.e.~all of the weights in a layer getting pruned. Figure \ref{fig:compare_purining_C10_3} visualizes the fraction of unpruned weights in input and output layers for various $\la$. HP (solid) curves are stable whereas MP (dotted) curves are highly volatile and easily hit zero except a narrow region. We note that, an alternative way of avoiding layer death is pruning layers individually. Supplementary provides further experiments on this for completeness.% we also conduct layer-wise pruning and observe that HP outperforms MP in both global and layer-wise pruning. 
\mc{didn't find layer death reference -Line 263}
%, we compute $\ix=\arg\min_{|\ix|=s}{\Ic_\ix(\bt_\fn)}$ for both MI and HI and hard prune the initial weights $\bt_{0}$ of the 2-layer network according to $\ix$.  Then we retrain the pruned network $\Pi_s(\bt_0)$ using same training data on cross entropy loss. Fig.~\ref{fig:compare_purining_C10_1} shows that MP fails immediately when $\lambda$ becomes smaller or larger because MP prunes the whole input or output layer due to the imbalanced MI between layers. But HP in Fig.~\ref{fig:compare_purining_C10_2} is resilient to layer scaling because reweighing using hessian matrix preserves the importance ratio among layers. We remark that we also conduct layer-wise pruning and observe that HP outperforms MP in both global and layer-wise pruning. The additional results are attached in appendix. The following theorem will demystify the advantage of HP in an analytical way.

%In short, small weights stay small.

%$\W$ and $\V$ are preserved.
 %and HI after training is slightly scaled w.r.t. $\lambda$ in both Fig.~\ref{fig:Importance_layer_1} and \ref{fig:Importance_layer_2}, but  
 
 %over-parameterized shallow network, since 
 %dominates the training when they are competing between each other for fitting.
 \vs
\noindent{\bf{Understanding NI and optimization dynamics:}} If our shallow network is sufficiently wide, each layer (or large groups of weights) can individually fit the training dataset. This can be viewed as a competition between the layers and a natural question is how much a layer contributes to the learning. This question is answered by NI. In Figure \ref{fig:Importance_layer_1} orange line displays the change in input layer NI (with $\Lc$ of Def.~\ref{def: weight impo} is training loss) which demonstrates that NI is decreasing function of $\la$ and moves in the opposite direction to MI. Figure \ref{fig:Importance_layer_test} verifies the same NI behavior for test loss and test error. Specifically, for large $\la$, input layer is responsible for most of the test accuracy and for small $\la$, it is the output layer. \mc{"it is the output layer" seems a bit strange, can we change to "output layer takes the role" --Line 273/274} Our key technical contribution in this section is {\em{providing a theoretical explanation to this NI behavior and relating it to optimization dynamics}}. In essence, we will connect NI to the only feature in Lemma \ref{simple hessian gradient} that exhibit similar behavior, the Hessian. Below we state our result on the Hessian and NI relation in terms of Polyak-Lojasiewicz (PL) condition \cite{karimi2016linear}.

% NI provide an evidence that the layer with smaller weights gains more importance in Fig.~\ref{fig:Importance_layer_1} and \ref{fig:Importance_layer_2} which is in contrast to MI. One explanation is that in this setup the layer with smaller weights has larger gradient which leads to the larger contribution while training. It directly connects the intuition of Thm.~\ref{lem win} which states that weights with larger gradient in training gain more importance.

%without requiring weights to significantly change.


% coincide and with $\la$ and $\la^{-1}$. Lemma \ref{simple hessian gradient} explains the initial behavior. The final beha

 


%\som{This section focuses on magnitude pruning. Note that pruning each layer to a certain fraction of nonzeros might circumvent the issue of killing whole layer. However, in appendix, we also verified that regular hessian pruning works better than both layerwise MP and HP}




\begin{figure}[t!]
	\begin{subfigure}{1.78in}\vspace{-5pt}
		\centering
		\begin{tikzpicture}
		\node at (0,0) {\includegraphics[scale=0.325]{figs/Importance_layer_1}};
		\node at (-2.4,0) [rotate=90,scale=.9]{Importance};
		\node at (0,-1.7) [scale=.9]{$\lambda$};%Each bar in the figure shows the correlations' geometric mean of datasets in this group when training to corresponding non-zero level. 
		\end{tikzpicture}\caption{\small{Importance of input layer $\W_\fn^\la$}}\label{fig:Importance_layer_1}\vspace{-0.2cm}
	\end{subfigure}~\begin{subfigure}{1.78in}\vspace{-5pt}
	\centering
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.325]{figs/Importance_layer_2}};
	%\node at (-2.4,0) [rotate=90,scale=.7]{Importance};
	\node at (0,-1.7) [scale=.9]{$\lambda$};%Each bar in the figure shows the correlations' geometric mean of datasets in this group when training to corresponding non-zero level. 
	\end{tikzpicture}\caption{\small{Importance of output layer $\V_\fn^\la$}}\label{fig:Importance_layer_2}\vspace{-0.2cm}
\end{subfigure}\begin{subfigure}{1.78in}\vspace{-5pt}
\centering
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.325]{figs/Importance_layer_test}};
	%\node at (-2.4,0) [rotate=90,scale=.7]{Loss or Accuracy};
	\node at (0,-1.7) [scale=.9]{$\lambda$};%Each bar in the figure shows the correlations' geometric mean of datasets in this group when training to corresponding non-zero level. 
	\end{tikzpicture}\caption{\small{Natural importances w.r.t.~test}}\label{fig:Importance_layer_test}\vspace{-0.2cm}
\end{subfigure}\caption{\small{(a) and (b) show the comparison of importance criterias for input and output layers when training with a shallow network with cross entropy and with initializations $\bt_\ini^\la=(\la\W_\ini,\la^{-1}\V_\ini)$. (c) shows the NI w.r.t.~test classification error and loss obtained by setting one of the layers to its initialization. }}\label{fig:Importance_layer}\vspace{-15pt}
\end{figure}
%We remark that we use soft pruning whose reference weights $\bt_R=\bt_0$ to access each layer's NI. 

\vs\begin{definition}[Partial PL and Smoothness (PPLS)] Let $\Lc(\bt)$ be a loss function satisfying $\min_{\bt}\Lc(\bt)=0$. Given an index set $\Delta\subset[p]$, we say that PPLS holds with parameter $L\geq \mu\geq 0$ if partial derivative $\frac{\pa }{\pa \bt_{\Delta}}\Lc(\bt)$ is $L$-Lipschitz function of $\bt_{\Delta}$ and obeys $\tn{\frac{\pa }{\pa \bt_{\Delta}}\Lc(\bt)}^2\geq 2\mu\Lc(\bt)$.
%\[
%\tn{\frac{\pa }{\pa \bt_{\Delta}\Lc(\bt)}}^2\geq 2\mu_\Delta\Lc(\bt).
%\]
\end{definition}\vs
While PL allows for non-convex optimization, when specialized to strong convexity, Partial PL condition provides a lower bound on the submatrix of Hessian induced by the set $\ix$. Regular PL condition guarantees global convergence of gradient descent, thus if PPLS holds over $\ix$, training only over $\ix$ is sufficient to achieve zero loss. A good example of PPLS is linear regression with two feature sets $\X_1\in\R^{n\times p_1}$ and $\X_2\in\R^{n\times p_2}$ with $p_1,p_2\geq n$ where we fit \mc{ to be consist, dim of X1 and X1 should be d1 d2? I feel both are ok but which is better?}
\begin{align}
\Lc(\bt)=\min_{\bt=[\bt_1~\bt_2]}0.5\tn{\y-\X_1\bt_1-\X_2\bt_2}^2.\label{lin reg}
\end{align}
$\Lc$ satisfies PPLS over $[p_1]=\{1,\dots,p_1\}$ with parameters $L_1=\|\X_1\|^2$ and $\mu_1=\sigma_{\min}(\X_1)^2$. For randomly initialized over-parameterized networks, each layer solves a kernel regression and would satisfy PPLS under mild conditions on the dataset \cite{chizat2019lazy,du2018gradient,jacot2018neural,allen2019convergence} \mc{also \cite{lee2019wide}} . Specifically, linearized neural network dynamics on $\bt=(\W,\V)$ connects \mc{connects-> connect} to the regression task \eqref{lin reg} via the Taylor expansion around initialization where input and output layers have linearized features arising from the Jacobian map given by $\X_{\W}=[\frac{\pa f(\x_1)}{\pa \W}~\dots~\frac{\pa f(\x_n)}{\pa \W}]^T\in\R^{n\times md}$ and $\X_{\V}=[\frac{\pa f(\x_1)}{\pa \V}~\dots~\frac{\pa f(\x_n)}{\pa \V}]^T\in\R^{n\times Km}$. The following theorem provides a theoretical explanation of NI behavior via PPLS by quantifying relative contributions of different sets of weights.
\vs
\mc{ added arrow for fig 3a, adjusted size of 3c} 
\begin{theorem}[Larger Hessian Wins More]\label{lem win}
Suppose the entries of $\bt\in\R^p$ are union of $D$ non-intersecting sets $(\Delta_i)_{i=1}^D\subset [p]$ and PPLS holds over $\ix_i$ with parameters $L_i\geq \mu_i\geq 0$ for all $i$. Set $\mu=\sum_{i=1}^D\mu_i$ and $L=\sum_{i=1}^DL_i$. Starting from a point $\bt_0$, and using a learning rate $\eta\leq 1/L$, run gradient iterations $\bt_{\tau+1}=\bt_\tau-\eta \grad{\bt_\tau}$. For all iterates $\tau$, the loss obeys $\Lc(\bt_\tau)\leq (1-\eta\mu)^\tau \Lc(\bt_0)$. Furthermore, setting $\kappa=L_i/\mu$, the following bounds hold for $\iii$ and $\iib=[p]-\iii$ for all $\tau\geq 0$
\begin{align}
&\tn{\bt_{\iii,\tau}-\bt_{\iii,0}}^2\leq 8{\kappa}\Lc(\bt_0)/\mu,\label{dist bound}\\
&{\Icn_{\iii}(\bt_\tau,\bt_0)}/{\Lc(\bt_0)}\leq 8\kappa^2+4{\kappa}(1-\eta\mu)^{\tau/2},\label{bad2}\\%\Lc(\bt_0)(L_I/\mu+(L/\mu+1)(1-\eta\mu)^{\tau/2}).
&{\Icn_{\iib}(\bt_\tau,\bt_0)}/{\Lc(\bt_0)}\geq 1-8\kappa^2-4{\kappa}-(1-\eta\mu)^\tau\label{good2}.
\end{align}
\end{theorem}\vs%In words, this result upper 
In words, this theorem captures the NI of a subset of weight\mc{weight->weights} throughout the training via the upper and lower bounds \eqref{bad2} and \eqref{good2}. For the experiments in Fig.~\ref{fig:Importance_layer}, based on \eqref{gradient change} of Lemma \ref{simple hessian gradient}, PPLS parameters $(\mu_{\W},L_{\W})$ of the input layer decay as $\la^{-2}$ and output layer parameters grow as $\la^2$. Thus, assuming $\la\geq 1$, for output layer we have $\kappa=L_{\W}/(\mu_{\W}+\mu_{\V})\sim \la^{-4}$ and, using \eqref{bad2} with $\tau=\infty$, NI is expected to decay as $\kappa^2\sim\la^{-8}$ (e.g.~for quadratic loss). Similarly, NI of the input layer is lower bounded via \eqref{good2} which grows as $1-{\cal{O}}(\la^{-4})$. Finally, for small $\la$, we have the reversed upper/lower bounds. In summary, our Theorem \ref{lem win} successfully explains the empirical NI behavior in Fig.~\ref{fig:Importance_layer}.



\vs
\eqref{dist bound} generalizes the ``short distance from initialization'' results of \cite{oymak2018overparameterized} by controlling individual subsets of weights and also provides a bound on MI when $\bt_0=0$. As explained in supplementary, {\em{this theorem is tight up to local ($L_i/\mu_i$) and global ($L/\mu$) condition numbers and accurately captures the relative contributions of the weights $(\bt_{\iii})_{i=1}^D$}}. Observe that this theorem considers the Init-Pruning (w.r.t.~$\bt_0$) which is better suited for assessing optimization dynamics.

Note that the bounds of Thm \ref{lem win} greatly simplify at the global minima ($\tau\rightarrow\infty$). As mentioned earlier, training NI of Figure \ref{fig:covariance} can be explained by Thm~\ref{lem win}. In essence, scaling up a set of features increase their covariance (and PPLS parameter $\mu$) increasing the NI w.r.t.~training loss.

% as a function of $\la$
%\noindent{\bf{Case study -- Neural Net NI:}} 





%In short, Hessian structure leads to larger gradients
%when $\la$ decays, the NI behavior is flipped.
%
%Suppose $n=1$ and we have $\Lc(\bt)=0.5(y-\x^T\bt)^2$. $\bt_\st=y\x/\tn{\x}^2$. $L_i=\mu_i=|\x_i|^2$, $\mu=\tn{\x}^2$.
%
%\[
%(y-y\x_1^2/\tn{\x}^2)^2=\Lc(\bt_0)(1-\x_1^2/\tn{\x}^2)^2=\Lc(\bt_0)(1-L_1/\mu)^2=(1-2\sqrt{\kappa}+\kappa)
%\]
%\[
%\X,\y\implies \X^\dagger\y=\X^T(\X\X^T)^{-1}\y\quad \tn{\bt_{\iii}}\geq \sigma_{\min}(\X_i)\frac{1}{\|\X\|^2}\tn{\y}\geq \sqrt{\mu_i}\sqrt{\Lc(\bt_0)}/L
%\]
%\begin{theorem}[Larger Gradient Wins More]\label{lem win}
%Suppose entries of $\bt$ are composed of two non-intersecting sets $\ixf,\ixs\subset [p]$. Suppose $\Lc$ is $L$-smooth and PPLS holds over $\ixf$ with parameters $L_1\geq \mu_1$ and over $\ixs$ with $L_2\geq \mu_2$. Set $\kappa=L_1/\mu_2$ and $\mu=\mu_1+\mu_2$. Starting from a point $\bt_0$, and using a learning rate $\eta\leq 1/L$, run gradient iterations
%\[
%\bt_{\tau+1}=\bt_\tau-\eta \grad{\bt_\tau}.
%\]
%For all iterates $\tau$, the loss obeys $\Lc(\bt_\tau)\leq (1-\eta\mu)^\tau \Lc(\bt_0)$ and we have the following NI bounds
%\begin{align}
%\Icn_{\ixf}{(\bt_\tau,\bt_0)}/{\Lc(\bt_0)}&\leq 8\kappa+4\sqrt{\kappa}(1-\eta\mu)^{\tau/2},\label{good}\\
%\Icn_{\ixs}{(\bt_\tau,\bt_0)}/\Lc(\bt_0)&\geq 1-8\kappa-4\sqrt{\kappa}-(1-\eta\mu)^\tau.\label{bad}%\Lc(\bt_0)(L_I/\mu+(L/\mu+1)(1-\eta\mu)^{\tau/2}).
%\end{align}
%\end{theorem}

\begin{comment}
The main message of the theorem above is most visible when we let $\tau\rightarrow \infty$ and when the PL growth parameter $\mu_2$ of $\ixs$  dominates the Lipschitz constant $L_1$ of $\ixf$ i.e.~$\mu_2/L_1=\kappa^{-1}\gg 1$. Under this condition, the NI of $\bt_\ixf$ is relatively small so removing the progress made by $\bt_\ixf$ only mildly hurts the performance as the loss increasing is at most $8\kappa \Lc(\bt_0)$. In contrast, removing the contribution of $\bt_\ixs$ increases the loss proportional to $\sqrt{\kappa}$. 

For a case study, considering the model defined by \ref{loss}, let $L_{\W}$, $\mu_{\W}$, $L_{\V}$, $\mu_{\V}$ denotes the PPLS condition for $\ixi$, $\ixo$, and define $\kappa=L_{\W_0}/\mu_{\V_0}$, $\kappa'=L_{\V_0}/\mu_{\W_0}$. When assuming $\tau\rightarrow \infty$ and $\ixf=\ixi$, $\ixs=\ixo$, with $\lambda$-scaling, we have $\mu_{\V^\la}=\la^2\mu_{\V_0}$ and $L_{\W^\la}=\la^{-2}L_{\W_0}$ via \ref{gradient change}, and $\kappa_\lambda=L_{\W^\la}/\mu_{\V^\la}=\la^{-4}\kappa$. On the other hand, since $\ixf$ and $\ixs$ are interchangeable, when assuming $\ixf=\ixo$, $\ixs=\ixi$, we induce $\kappa_\la'=\la^4\kappa'$. Applying Thm.~\ref{lem win}, we have

$$1-8\la^4\kappa'-4\la^2\sqrt{(\kappa')}\leq\Icn_{\ixi}{(\bt_\tau^\la,\bt_0^\la)}/{\Lc(\bt_0^\la)}\leq 8\la^{-4}\kappa.$$

So the increase in  $\lambda$ leads to the decrease of $\Icn_{\ixi}{(\bt_\tau^\la,\bt_0^\la)}/{\Lc(\bt_0^\la)}$ which coincides with the orange line in Fig.~\ref{fig:Importance_layer_1}. 

Going back to the least-squares problem \eqref{eqn: ERM linear} and $\lambda$-scaling on linear problem \eqref{linear scaling}. Since we discussed HI and NI coincides for linear model, Thm.~\ref{lem win} is able to applied to predict performance for linear model when solving with gradient method. In each update, gradient can be written as $g_\Lambda=1/n\sum_{i=1}^{n}{\x^{\Lambda\top}(y_i-\hat{y}_i)}$ where $\hat{y}$ is the model prediction. Thus, for weight entries with $\lambda$ scaling, since the gradient of these entries is scaled by lambda, the NI also scaled by $\la$, which leads to the experiment results in Fig.~\ref{fig:positive} and \ref{fig:negative}. In, fig.~\ref{fig:covariance}, comparing to the blue line where $\la=1$, increasing $\la$ directly enhance the NI of first $s$ entries (the red line), and decreasing $\la$ leads to the decrease in NI.
\end{comment}

%For the neural network, recent literature \cite{jacot2018neural,su2019learning,du2019gradient,chizat2019lazy,oymak2019towards,zou2018stochastic} indicate that Jacobian feature map $\Jb(\bt)=\frac{\pa f(\bt)}{\pa \bt}\in\R^{n\times p}$ acts as an ``instantaneous'' design matrix and governs the optimization dynamics via the first order approximation
%\begin{align}
%f(\bt+\Delta)\approx f(\bt)+\Jb(\bt)\Delta.\label{nn jacob}
%\end{align}
%This approximation is also at the core of the recent works on Neural Tangent Kernel \cite{jacot2018neural,du2018gradient}. Another line of literature\cite{jacot2018neural,zou2018stochastic,lee2019wide} shows that in extremely wide or infinite wide neural networks, the weights move slowly from initialization.  Hence, properties of $\Jb$ may dictate which weights have a stronger say in the network's decision than others. 

%suppose $\X_2$ is weaker than $\X_1$ in the sense that $\sigma_{\min}(\X_1)\gg \|\X_2\|$. This implies $\mu\gg L_2$, since for linear regression \eqref{LS}, it can be shown that, $\mu =\sigma^2_{\min}(\X)\geq \sigma^2_{\min}(\X_1)$ and $L_2=\|\X_2\|^2$. Thus, gradient descent will prefer $\X_1$ over $\X_2$ and most of the prediction of the final model will be due to $\X_1$. While Theorem \ref{lem win} considers possibly non-convex problems, Appendix C provides further insights on how modifying the feature strength via scaling affect the solutions of the linear problem \eqref{LS}.%monotonic behavior of fe
% if the spectrum of the problem is aligned with prominent features, 
%Secondly, we will  why feature selection is possible without explicit sparsity regularization. 

%Indeed to obtain good solutions such explicit regularization is often crucial to have any chance of success.

\begin{figure}[t!]
	\begin{subfigure}{1.78in}
		\centering
		\begin{tikzpicture}[scale=1,every node/.style={scale=1}]
		\node at (0,0) {\includegraphics[scale=0.32]{figs/retrain_naive_acc.pdf}};
		\node at (-2.3,0) [rotate=90,scale=.7]{Test accuracy};
		\node at (0,-1.7) [scale=.7]{Fraction of non-zero};
		\node at (-1.1,-0.7) [scale=.6] {$\V=0$};
		\node at (1.1,-0.7) [scale=.6] {$\W=0$};
		\draw [->,>=stealth] (-1.2,-0.8) -- (-1.45,-0.95);
		\draw [->,>=stealth] (1.1,-0.8) -- (0.85,-0.95);
		%\node at (2.4,0) [rotate=90,scale=.8]{$\log_{10}{\lambda}$};
		\end{tikzpicture}\caption{\small{Test accuracy using MP. }}\label{fig:compare_purining_C10_1}
	\end{subfigure}\begin{subfigure}{1.78in}
		\centering
		\begin{tikzpicture}[scale=1,every node/.style={scale=1}]
		\node at (0,0) {\includegraphics[scale=0.32]{figs/retrain_jacobian_acc.pdf}};
		\node at (-2.3,0) [rotate=90,scale=.7]{Test accuracy};
		\node at (0,-1.7) [scale=.7]{Fraction of non-zero};
		
		%\node at (2.4,0) [rotate=90,scale=.8]{$\log_{10}{\lambda}$};
		\end{tikzpicture}\caption{\small{Test accuracy using HP.}}\label{fig:compare_purining_C10_2} 
	\end{subfigure}\begin{subfigure}{1.78in}
		\centering\vspace{6pt}
		\begin{tikzpicture}[scale=1,every node/.style={scale=1}]
		\node at (0,0) {\includegraphics[scale=0.29]{figs/width_init.pdf}};
		\node at (-2.25,0) [rotate=90,scale=.7]{Remaining output layer };
		\node at (2.3,0) [rotate=90,scale=.7]{Remaining input layer };
		\node at (0,-1.6) [scale=.7]{$\lambda$};
		%\node at (2.4,0) [rotate=90,scale=.8]{$\log_{10}{\lambda}$};
		\end{tikzpicture}\caption{\small{Remaining nonzeros for $\V,\W$}}\label{fig:compare_purining_C10_3} 
	\end{subfigure}\caption{\small{In (a) and (b), we first apply MP and HP on the network weights $\bt_\fn^{(\la)}$ for varying pruning levels $s/p$ where $p=(K+d)m$. We then retrain the pruned network from same initial nonzeros (lottery initialization of \cite{frankle2019lottery}) and display the test accuracy. HP is more stable compared to MP under $\la$-scaled initializations. (c) Visualization of the remaining fractions of nonzero weights in input (red) and output (blue) layers after pruning the network to 1\% sparsity. Nonzero counts in both layers are stable under HP but rapidly change in MP as a function of $\la$.}}\label{fig:compare_pruning_C10}\vspace{-12pt}
	% In Fig.~\ref{fig:compare_purining_C10_1} and \ref{fig:compare_purining_C10_2}, we firstly compute $\ix=\arg\min_{|\ix|=s}{\Ic_\ix(\bt_\fn)}$ for both MI and HI and hard prune the initial weights $\bt_{0}$ of the 2-layer network $f(\x)=\text{Softmax}(\V\text{ReLu}(\W\x))$ according to $\ix$.  Then we retrain the pruned network $\Pi_s(\bt_0)$ using same training data and cross entropy loss. Fig.~\ref{fig:compare_purining_C10_1} shows that only $\lambda=1$ survives during MP because weights magnitudes are balanced between two layers. However, when $\la$ becomes larger, the output layer $\V$ is completely pruned which leads to the red and blue lines in Fig.~\ref{fig:compare_purining_C10_1}. And when $\la$ becomes smaller the input layer $\W$ will be totally pruned when the model become extremely sparse. Fig.~\ref{fig:compare_purining_C10_2} shows that HP out performs MP especially in extremely sparse regime and .} }\label{fig:compare_purining_C10}\vspace{-12pt}
\end{figure}


==> neuralnet_bc.tex <==

\section{Gradient Bias and the Role of Initialization for Neural Nets}\label{neural sec}
%So far we discussed pruning and implicit bias in linear models. 
This section extends our discussion of importance and pruning to another fundamental model class: neural networks with one-hidden layer. Suppose output dimension is $K$ and the network has $m$ hidden units. Such a network with ReLU activation is given by $f_{\bt}(\x)=\V\act{\W\x}$, where $\W\in\R^{m\times p}$ and $\V\in\R^{K\times m}$ are the input and output layers respectively and $\bt=(\W,\V)\in\R^{(p+K)m}$ is the vector composed of the entries of $\W,\V$. Let $\ixi$ and $\ixo$ denote the index of the entries of $\W,\V$ in $\bt$. Given a dataset $(\x_i,y_i)_{i=1}^n$ and loss $\ell$, we minimize% the loss
\begin{align}
\Lc(\bt)=\frac{1}{n}\sum_{i=1}^n\ell(y_i,f_{\bt}(\x_i)).\label{loss}
\end{align}
{\bf{Equivalent networks:}} To study neural net pruning and initialization, we shall consider a class of networks $\bt^\la=(\la\W_0,\la^{-1}\V_0)$ generated from a base network $\bt^1=(\W_0,\V_0)$. Observe that all vectors $\bt^\la$ implement the same function due to the linearity of ReLU however magnitudes of layers are varying. The following lemma shows how the parameter $\la$ affects MI, HI, and gradient.
%Throughout this section, we will focus on shallow neural networks of the form $f_{\bt}(\x)=\V\act{\W\x}$ where $\bt\in\R^{}$ is the vector composed of the entries of input layer $\W$ and output layer $\V$. \dots
\begin{lemma} \label{simple hessian gradient}Consider the loss \eqref{loss}. For all $\la>0$, HI and partial derivatives obey%\som{Consider removing MI which is trivial}
%[Importance -- Shallow Network] 
\begin{align}
&\Ic^M_\ixi(\bt^\la)=\la\Ic^M_\ixi(\bt^1)\quad\text{and}\quad\Ic^M_\ixo(\bt^\la)=\la^{-1}\Ic^M_\ixo(\bt^1),\nn\\
&\Ic^H_\ixi(\bt^\la)=\Ic^H_\ixi(\bt^1)\quad\text{and}\quad\Ic^H_\ixo(\bt^\la)=\Ic^H_\ixo(\bt^1),\label{constant HI}\\
&\nabla_{\W}\Lc(\bt^\la)=\la^{-1}\nabla_{\W}\Lc(\bt^1)\quad\text{and}\quad\nabla_{\V}\Lc(\bt^\la)=\la\nabla_{\V}\Lc(\bt^1).\label{gradient change}
\end{align}
\end{lemma}
In words, increasing $\la$ increases MI, preserves HI, and decreases the gradient magnitude for the input layer and has the reverse affect on the output layer. Suppose we train the network from initializations $\bt^\la$ on \eqref{loss}. What happens at the end of the training as a function of $\la$? Does eventual MI and HI exhibit similar behavior to initialization? What about NI?

% in training
To answer these, let us first introduce the related notation. Let $\bt_\fn^\la=(\la\W_\fn,\la^{-1}\V_\fn)$ denote the  final model after training to fit, and $\W_\fn^\la=\la\W_\fn$, $\V_\fn^\la=\la^{-1}\V_\fn$ be the shorthand notation to represent the weights of each layer under $\la$-scaling. In Fig.~\ref{fig:Importance_layer_1} and \ref{fig:Importance_layer_2}, we train a one-hidden layer network with cross entropy loss on MNIST. Here $m=1024$, $p=784$ and $K=10$. We set $\bt^{1}_{0}=(\W_0,\V_0)$ with \textit{He normal} initialization \cite{he2015delving}. We then train new networks with $\la$-scaled initializations $\bt^\la_0=(\la\W_0,\la^{-1}\V_0)$ via factor $\lambda$, we show the dynamic of MI,HI,NI for $\W$ and $\V$ in Fig.~\ref{fig:Importance_layer_1},~\ref{fig:Importance_layer_2} respectively. Specially, we remark that to enforce that all lines are in the same range for better plots, we draw the green line for $10^5$HI instead of original HI. The orange lines (HI) in Fig.~\ref{fig:Importance_layer_1},~\ref{fig:Importance_layer_2} are results of soft pruning where we replace $\W_\fn^\la$ to $\W_0^\la$ in Fig.~\ref{fig:Importance_layer_1} and $\V_\fn^\la$ to $\V_0^\la$ in Fig.~\ref{fig:Importance_layer_2}. In Fig.~\ref{fig:Importance_layer_1} and \ref{fig:Importance_layer_2}, both initial and final MI exactly coincide with $\la$. Furthermore, the initial HI stays constant which coincide with Lemma~\ref{simple hessian gradient} and HI after training is slightly scaled w.r.t. $\lambda$ in both Fig.~\ref{fig:Importance_layer_1} and \ref{fig:Importance_layer_2}, but the ratio of HI between $\W$ and $\V$ are preserved. Moreover, for this over-parameterized shallow neural network, since each layer is able to fit all training samples, it raises a question that which layer can dominate the training when they are competing between each other for fitting. Then NI provide an evidence that the layer with smaller weights gains more importance in Fig.~\ref{fig:Importance_layer_1} and \ref{fig:Importance_layer_2} which is in contrast to MI. One explanation is that in this setup the layer with smaller weights has larger gradient which leads to the larger contribution while training. It directly connects the intuition of Thm.~\ref{lem win} which states that weights with larger gradient in training gain more importance.

Moreover, In Fig.~\ref{fig:compare_purining_C10_1} and \ref{fig:compare_purining_C10_2}, we compute $\ix=\arg\min_{|\ix|=s}{\Ic_\ix(\bt_\fn)}$ for both MI and HI and hard prune the initial weights $\bt_{0}$ of the 2-layer network according to $\ix$.  Then we retrain the pruned network $\Pi_s(\bt_0)$ using same training data on cross entropy loss. Fig.~\ref{fig:compare_purining_C10_1} shows that MP fails immediately when $\lambda$ becomes smaller or larger because MP prunes the whole input or output layer due to the imbalanced MI between layers. But HP in Fig.~\ref{fig:compare_purining_C10_2} is resilient to layer scaling because reweighing using hessian matrix preserves the importance ratio among layers. We remark that we also conduct layer-wise pruning and observe that HP outperforms MP in both global and layer-wise pruning. The additional results are attached in appendix. The following theorem will demystify the advantage of HP in an analytical way. 


\som{This section focuses on magnitude pruning. Note that pruning each layer to a certain fraction of nonzeros might circumvent the issue of killing whole layer. However, in appendix, we also verified that regular hessian pruning works better than both layerwise MP and HP}




\begin{figure}[t!]
	\begin{subfigure}{1.78in}\vspace{-5pt}
		\centering
		\begin{tikzpicture}
		\node at (0,0) {\includegraphics[scale=0.325]{figs/Importance_layer_1}};
		\node at (-2.4,0) [rotate=90,scale=.7]{Importance};
		\node at (0,-1.7) [scale=.7]{$\lambda$};%Each bar in the figure shows the correlations' geometric mean of datasets in this group when training to corresponding non-zero level. 
		\end{tikzpicture}\caption{\small{Importance of $\W$ when scaling layer's initialization $\W=\lambda\W_0$.\\\quad\quad}}\label{fig:Importance_layer_1}\vspace{-0.2cm}
	\end{subfigure}\begin{subfigure}{1.78in}\vspace{-5pt}
	\centering
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.325]{figs/Importance_layer_2}};
	\node at (-2.4,0) [rotate=90,scale=.7]{Importance};
	\node at (0,-1.7) [scale=.7]{$\lambda$};%Each bar in the figure shows the correlations' geometric mean of datasets in this group when training to corresponding non-zero level. 
	\end{tikzpicture}\caption{\small{Importance of $\V$ when scaling layer's initialization $\V=\lambda^{-1}\V_0$.\\\quad\quad}}\label{fig:Importance_layer_2}\vspace{-0.2cm}
\end{subfigure}\begin{subfigure}{1.78in}\vspace{-5pt}
\centering
	\begin{tikzpicture}
	\node at (0,0) {\includegraphics[scale=0.325]{figs/Importance_layer_test}};
	%\node at (-2.4,0) [rotate=90,scale=.7]{Loss or Accuracy};
	\node at (0,-1.7) [scale=.7]{$\lambda$};%Each bar in the figure shows the correlations' geometric mean of datasets in this group when training to corresponding non-zero level. 
	\end{tikzpicture}\caption{\small{Test error and loss when setting $\W_\fn$ and $\V_\fn$ to $\W_0$ and $V_0$ respectively under scaling $\lambda$.}}\label{fig:Importance_layer_test}\vspace{-0.2cm}
\end{subfigure}\caption{\small{Fig.~\ref{fig:Importance_layer_1} and \ref{fig:Importance_layer_2} show the comparison of various importance measurements for input and output layers when training on two layer network $f(\x)=\text{Softmax}(\V\text{ReLu}(\W\x))$ with cross entropy loss on MNIST where $\W\in\R^{1024\times784}$ and $\V\in\R^{10\times1024}$ with initialization $\bt^\la=(\la\W_0,\la^{-1}\V_0)$, where $\W_0$, $\V_0$ are initialized by \textit{He normal}\cite{he2015delving}. We remark that we use soft pruning whose reference weights $\bt_R=\bt_0$ to access each layer's NI. Fig.~\ref{fig:Importance_layer_test} shows the test error and loss when replacing one layer to its initialization where solid lines replace $\V_\fn^\la$ by $\V_0^\la$ and dash lines replace $\W_\fn^\la$ by $\W_0^\la$. }}\label{fig:Importance_layer}\vspace{-12pt}
\end{figure}



\begin{definition}[Partial PL and Smoothness (PPLS)] Let $\Lc(\bt)$ be a loss function satisfying $\min_{\bt}\Lc(\bt56)=0$. Given an index set $\Delta\subset[p]$, we say that PPLS holds with parameter $L\geq \mu\geq 0$ if partial derivative $\frac{\pa }{\pa \bt_{\Delta}}\Lc(\bt)$ is $L$-Lipschitz function of $\bt_{\Delta}$ and obeys $\tn{\frac{\pa }{\pa \bt_{\Delta}}\Lc(\bt)}^2\geq 2\mu\Lc(\bt)$.
%\[
%\tn{\frac{\pa }{\pa \bt_{\Delta}\Lc(\bt)}}^2\geq 2\mu_\Delta\Lc(\bt).
%\]
\end{definition}
In words, if PPLS holds over $\ix$, training only over $\ix$ is sufficient to achieve zero loss.

\begin{theorem}[Larger Gradient Wins More]\label{lem win}
Suppose the entries of $\bt$ are union of $D$ non-intersecting sets $(\Delta_i)_{i=1}^D\subset [p]$ and PPLS holds over $\ix_i$ with parameters $L_i\geq \mu_i\geq 0$ for all $i$. Set $\mu=\sum_{i=1}^D\mu_i$ and $L=\sum_{i=1}^DL_i$. Starting from a point $\bt_0$, and using a learning rate $\eta\leq 1/L$, run gradient iterations $\bt_{\tau+1}=\bt_\tau-\eta \grad{\bt_\tau}$. For all iterates $\tau$, the loss obeys $\Lc(\bt_\tau)\leq (1-\eta\mu)^\tau \Lc(\bt_0)$. Furthermore, setting $\kappa=(L_i/\mu)^2$, the following bounds hold for $\iii$ for all $\tau\geq 0$
\begin{align}
&\tn{\bt_{\iii,\tau}-\bt_{\iii,0}}^2\leq 8\sqrt{\kappa}\Lc(\bt_0)/\mu,\label{dist bound}\\
&{\Icn_{\iii}(\bt_\tau,\bt_0)}/{\Lc(\bt_0)}\leq 8\kappa+4\sqrt{\kappa}(1-\eta\mu)^{\tau/2},\label{bad2}\\%\Lc(\bt_0)(L_I/\mu+(L/\mu+1)(1-\eta\mu)^{\tau/2}).
&{\Icn_{\iib}(\bt_\tau,\bt_0)}/{\Lc(\bt_0)}\geq 1-8\kappa-4\sqrt{\kappa}-(1-\eta\mu)^\tau,\label{good2}.
\end{align}
\end{theorem}
In words, this theorem captures the evolution of a weight subset throughout the training. In words, this result upper As explained in supplementary, this theorem is tight up to condition numbers $L_i/\mu_i,~L/\mu$. In other words, it captures the correct competition between the weights $(\bt_{\iii})_{i=1}^D$.
%
%Suppose $n=1$ and we have $\Lc(\bt)=0.5(y-\x^T\bt)^2$. $\bt_\st=y\x/\tn{\x}^2$. $L_i=\mu_i=|\x_i|^2$, $\mu=\tn{\x}^2$.
%
%\[
%(y-y\x_1^2/\tn{\x}^2)^2=\Lc(\bt_0)(1-\x_1^2/\tn{\x}^2)^2=\Lc(\bt_0)(1-L_1/\mu)^2=(1-2\sqrt{\kappa}+\kappa)
%\]
%\[
%\X,\y\implies \X^\dagger\y=\X^T(\X\X^T)^{-1}\y\quad \tn{\bt_{\iii}}\geq \sigma_{\min}(\X_i)\frac{1}{\|\X\|^2}\tn{\y}\geq \sqrt{\mu_i}\sqrt{\Lc(\bt_0)}/L
%\]
%\begin{theorem}[Larger Gradient Wins More]\label{lem win}
%Suppose entries of $\bt$ are composed of two non-intersecting sets $\ixf,\ixs\subset [p]$. Suppose $\Lc$ is $L$-smooth and PPLS holds over $\ixf$ with parameters $L_1\geq \mu_1$ and over $\ixs$ with $L_2\geq \mu_2$. Set $\kappa=L_1/\mu_2$ and $\mu=\mu_1+\mu_2$. Starting from a point $\bt_0$, and using a learning rate $\eta\leq 1/L$, run gradient iterations
%\[
%\bt_{\tau+1}=\bt_\tau-\eta \grad{\bt_\tau}.
%\]
%For all iterates $\tau$, the loss obeys $\Lc(\bt_\tau)\leq (1-\eta\mu)^\tau \Lc(\bt_0)$ and we have the following NI bounds
%\begin{align}
%\Icn_{\ixf}{(\bt_\tau,\bt_0)}/{\Lc(\bt_0)}&\leq 8\kappa+4\sqrt{\kappa}(1-\eta\mu)^{\tau/2},\label{good}\\
%\Icn_{\ixs}{(\bt_\tau,\bt_0)}/\Lc(\bt_0)&\geq 1-8\kappa-4\sqrt{\kappa}-(1-\eta\mu)^\tau.\label{bad}%\Lc(\bt_0)(L_I/\mu+(L/\mu+1)(1-\eta\mu)^{\tau/2}).
%\end{align}
%\end{theorem}

The main message of the theorem above is most visible when we let $\tau\rightarrow \infty$ and when the PL growth parameter $\mu_2$ of $\ixs$  dominates the Lipschitz constant $L_1$ of $\ixf$ i.e.~$\mu_2/L_1=\kappa^{-1}\gg 1$. Under this condition, the NI of $\bt_\ixf$ is relatively small so removing the progress made by $\bt_\ixf$ only mildly hurts the performance as the loss increasing is at most $8\kappa \Lc(\bt_0)$. In contrast, removing the contribution of $\bt_\ixs$ increases the loss proportional to $\sqrt{\kappa}$. 

For a case study, considering the model defined by \ref{loss}, let $L_{\W}$, $\mu_{\W}$, $L_{\V}$, $\mu_{\V}$ denotes the PPLS condition for $\ixi$, $\ixo$, and define $\kappa=L_{\W_0}/\mu_{\V_0}$, $\kappa'=L_{\V_0}/\mu_{\W_0}$. When assuming $\tau\rightarrow \infty$ and $\ixf=\ixi$, $\ixs=\ixo$, with $\lambda$-scaling, we have $\mu_{\V^\la}=\la^2\mu_{\V_0}$ and $L_{\W^\la}=\la^{-2}L_{\W_0}$ via \ref{gradient change}, and $\kappa_\lambda=L_{\W^\la}/\mu_{\V^\la}=\la^{-4}\kappa$. On the other hand, since $\ixf$ and $\ixs$ are interchangeable, when assuming $\ixf=\ixo$, $\ixs=\ixi$, we induce $\kappa_\la'=\la^4\kappa'$. Applying Thm.~\ref{lem win}, we have

$$1-8\la^4\kappa'-4\la^2\sqrt{(\kappa')}\leq\Icn_{\ixi}{(\bt_\tau^\la,\bt_0^\la)}/{\Lc(\bt_0^\la)}\leq 8\la^{-4}\kappa.$$

So the increase in  $\lambda$ leads to the decrease of $\Icn_{\ixi}{(\bt_\tau^\la,\bt_0^\la)}/{\Lc(\bt_0^\la)}$ which coincides with the orange line in Fig.~\ref{fig:Importance_layer_1}. 

Going back to the least-squares problem \eqref{eqn: ERM linear} and $\lambda$-scaling on linear problem \eqref{linear scaling}. Since we discussed HI and NI coincides for linear model, Thm.~\ref{lem win} is able to applied to predict performance for linear model when solving with gradient method. In each update, gradient can be written as $g_\Lambda=1/n\sum_{i=1}^{n}{\x^{\Lambda\top}(y_i-\hat{y}_i)}$ where $\hat{y}$ is the model prediction. Thus, for weight entries with $\lambda$ scaling, since the gradient of these entries is scaled by lambda, the NI also scaled by $\la$, which leads to the experiment results in Fig.~\ref{fig:positive} and \ref{fig:negative}. In, fig.~\ref{fig:covariance}, comparing to the blue line where $\la=1$, increasing $\la$ directly enhance the NI of first $s$ entries (the red line), and decreasing $\la$ leads to the decrease in NI.


For the neural network, recent literature \cite{jacot2018neural,su2019learning,du2019gradient,chizat2019lazy,oymak2019towards,zou2018stochastic} indicate that Jacobian feature map $\Jb(\bt)=\frac{\pa f(\bt)}{\pa \bt}\in\R^{n\times p}$ acts as an ``instantaneous'' design matrix and governs the optimization dynamics via the first order approximation
\begin{align}
f(\bt+\Delta)\approx f(\bt)+\Jb(\bt)\Delta.\label{nn jacob}
\end{align}
This approximation is also at the core of the recent works on Neural Tangent Kernel \cite{jacot2018neural,du2018gradient}. Another line of literature\cite{jacot2018neural,zou2018stochastic,lee2019wide} shows that in extremely wide or infinite wide neural networks, the weights move slowly from initialization.  Hence, properties of $\Jb$ may dictate which weights have a stronger say in the network's decision than others. 

%suppose $\X_2$ is weaker than $\X_1$ in the sense that $\sigma_{\min}(\X_1)\gg \|\X_2\|$. This implies $\mu\gg L_2$, since for linear regression \eqref{LS}, it can be shown that, $\mu =\sigma^2_{\min}(\X)\geq \sigma^2_{\min}(\X_1)$ and $L_2=\|\X_2\|^2$. Thus, gradient descent will prefer $\X_1$ over $\X_2$ and most of the prediction of the final model will be due to $\X_1$. While Theorem \ref{lem win} considers possibly non-convex problems, Appendix C provides further insights on how modifying the feature strength via scaling affect the solutions of the linear problem \eqref{LS}.%monotonic behavior of fe
% if the spectrum of the problem is aligned with prominent features, 
%Secondly, we will  why feature selection is possible without explicit sparsity regularization. 

%Indeed to obtain good solutions such explicit regularization is often crucial to have any chance of success. 
\begin{figure}[t!]
	\begin{subfigure}{1.78in}
		\centering
		\begin{tikzpicture}[scale=1,every node/.style={scale=1}]
		\node at (0,0) {\includegraphics[scale=0.32]{figs/retrain_naive_acc.pdf}};
		\node at (-2.3,0) [rotate=90,scale=.7]{Test accuracy};
		\node at (0,-1.7) [scale=.7]{Fraction of non-zero};
		\node at (-1.1,-0.7) [scale=.6] {$\V=0$};
		\node at (1.1,-0.7) [scale=.6] {$\W=0$};
		%\node at (2.4,0) [rotate=90,scale=.8]{$\log_{10}{\lambda}$};
		\end{tikzpicture}\caption{\small{Test accuracy using magnitude-based pruning (MP). \\}}\label{fig:compare_purining_C10_1}
	\end{subfigure}\begin{subfigure}{1.78in}
		\centering
		\begin{tikzpicture}[scale=1,every node/.style={scale=1}]
		\node at (0,0) {\includegraphics[scale=0.32]{figs/retrain_jacobian_acc.pdf}};
		\node at (-2.3,0) [rotate=90,scale=.7]{Test accuracy};
		\node at (0,-1.7) [scale=.7]{Fraction of non-zero};
		%\node at (2.4,0) [rotate=90,scale=.8]{$\log_{10}{\lambda}$};
		\end{tikzpicture}\caption{\small{Test accuracy using Hessian-based pruning (HP).\\}}\label{fig:compare_purining_C10_2} 
	\end{subfigure}\begin{subfigure}{1.78in}
		\centering
		\begin{tikzpicture}[scale=1,every node/.style={scale=1}]
		\node at (0,0) {\includegraphics[scale=0.32]{figs/width_init.pdf}};
		\node at (-2.3,0) [rotate=90,scale=.7]{Test accuracy};
		\node at (0,-1.7) [scale=.7]{Network width};
		%\node at (2.4,0) [rotate=90,scale=.8]{$\log_{10}{\lambda}$};
		\end{tikzpicture}\caption{\small{Test accuracy after retraining and 0.01 nonzero global pruning on various network widths when initializing with \textit{He normal}}}\label{fig:compare_purining_C10_3} 
	\end{subfigure}\caption{\small{In Fig.~\ref{fig:compare_purining_C10_1} and \ref{fig:compare_purining_C10_2}, we firstly compute $\ix=\arg\min_{|\ix|=s}{\Ic_\ix(\bt_\fn)}$ for both MI and HI and hard prune the initial weights $\bt_{0}$ of the 2-layer network $f(\x)=\text{Softmax}(\V\text{ReLu}(\W\x))$ according to $\ix$.  Then we retrain the pruned network $\Pi_s(\bt_0)$ using same training data and cross entropy loss. Fig.~\ref{fig:compare_purining_C10_1} shows that only $\lambda=1$ survives during MP because weights magnitudes are balanced between two layers. However, when $\la$ becomes larger, the output layer $\V$ is completely pruned which leads to the red and blue lines in Fig.~\ref{fig:compare_purining_C10_1}. And when $\la$ becomes smaller the input layer $\W$ will be totally pruned when the model become extremely sparse. Fig.~\ref{fig:compare_purining_C10_2} shows that HP out performs MP especially in extremely sparse regime and .} }\label{fig:compare_purining_C10}\vspace{-12pt}
\end{figure}


==> random_result.tex <==
\section{Improved $\ell_1$ Sample Complexity via Spectral Bias}\label{l1 improve}
%Recent decade witnessed immense progress in our understanding of linear inverse problems which lies at the core of compressed sensing. 

So far, we discussed the implicit bias of the plain gradient descent. $\ell_1/\ell_0$ regularization techniques are often critical for achieving state-of-the-art performance thus it is desirable to understand whether explicit and implicit regularization can synergistically facilitate feature selection. We shall answer this affirmatively by focusing on the sparse parameter recovery task ( via $\ell_1$ minimization) which has well-established sample complexity bounds under random design \cite{donoho2005sparse}. 

Suppose the input data is distributed as $(\x_i)_{i=1}^n\distas\Nn(0,\bSi)$ for some covariance matrix $\bSi\in\R^{p\times p}$. For the noiseless compressed sensing task, we assume that the labels are generated from an $s$ sparse ground-truth parameter $\bt_\st$ via the linear relation $y_i=\x_i^T\bt_\st$. The core quantity of interest is the number of samples required to recover the ground-truth parameter via the $\ell_1$ minimization problem
\begin{align}
\hat{\bt}_\st=\min_{\bt}\tone{\bt}\quad\text{subject to}\quad \X\bt=\X\bt_\st.\label{l1 prob}
\end{align}
Luckily, the rich compressed sensing literature has the answer for us for any choice of covariance matrix. The following lemma immediately follows from the seminal work of \cite{chandrasekaran2012convex} by applying a whitening trick and rewriting $\x^T\bt_\st=(\x^T\bSi^{-1/2})(\bSi^{1/2}\bt_\st)$ so that $\bSi^{-1/2}\x\distas\Nn(0,\Iden_p)$.%(\bt_\st^T\bSi^{1/2})(\bSi^{-1/2}\x)
\begin{lemma}[Gordon's lemma] \label{gordon sample}Define the tangent cone
\[
\Tc=\{\alpha \w\bgl \tone{\bt_\st+\w}\leq \tone{\bt_\st}\quad\text{and}\quad\alpha\geq 0\}.%\cap \Bc^{p}.
\]
Define the $\bSi$-colored Gaussian width to be
\[
\omega_{\bSi}(\Tc)=\E_{\g\sim\Nn(0,\Iden_p)}[\sup_{\w\in\bSi^{1/2}\Tc,\tn{\w}\leq 1}\g^T\w].
\]
If sample size satisfies $n\geq (\omega_{\bSi}(\Tc)+t)^2$, then with probability $1-\exp(-t^2/2)$, $\bt_\st$ is the unique solution of the $\ell_1$ problem \eqref{l1 prob}.
\end{lemma}
We remark that this result is tight and the success probability of the $\ell_1$ minimization exhibits a sharp phase transition around the Gaussian width threshold i.e.~$\ell_1$ minimization fails with high probability when $n< \omega^2_{\bSi}(\Tc)$ \cite{amelunxen2014living,oymak2017universality}. This tightness will allow us to capture the provable benefits of the spectral bias.% of the covariance.
%compressed sensing
%Classic compressed sensing  setup is when the inputs $\x_i$ are standard normal i.e.~$\x_i\distas\Nn(0,\Iden_p)$. Such unstructured inputs are a useful model for signal processing problems where the goal is collecting measurements of a signal $\bt_\st$.

The $\ell_1$ minimization phase transitions is well-studied for identity covariance and it is known that $2s\log(p/s)$ is a reasonable approximation to the sample complexity. For assessing spectral bias, we shall start with an intuitive spiked covariance model. Define the sign pattern of $\bt_\st$ (with entries $1,-1,0$) to be $\s=\sgn{\bt_\st}$. With this, we choose our sample covariance to be aligned with the sparse features as follows
\[
\E[\x\x^T]=\bSi_R\quad\text{where}\quad \bSi_R:=\Iden+\frac{R-1}{s}\s\s^T.%\Iden+(R-1)\s\s^T.
\]
Note that all eigenvalues of $\bSi_R$ are $1$ except the eigenvalue along the $\s$ direction which is equal to $R$. Can this spectral bias (when $R\geq 1$) help us push through the $\ell_1$ phase transitions? The next lemma answers this affirmatively by bounding the Gaussian width associated with $\bSi_R$ namely $\omega_R(\Tc):=\omega_{\bSi_R}(\Tc)$.% The next theorem establishes sample complexity bounds for recovering the $s$-sparse $\bt_\st$. 
\begin{lemma}\label{thm spike}Given $R\geq 1$, we have that%[Spiked Sample Complexity] 
\[
\omega_R^2(\Tc)\leq s(\frac{3}{2}+\frac{2\log(p/s)}{R^2}) \wedge (s(1+\frac{2\log(p)}{R^2})+1).
\]
\end{lemma}
%\noindent {\bf{Remark:}} For large $R$, $\omega_R$ will be made arbitrarily close to the degrees of freedom $s$ as the alternative bound $\omega_R(\Tc)\leq $ holds as well. 
This lemma shows that the required sample size becomes smaller as spectral bias $R$ increases. If we let $R\gg \sqrt{\log p}$, sample complexity drops to as little as $s$ which is the minimum number of equations required for {\em{exactly}} recovering the ground-truth $\bt_\st$. This result follows from a fairly standard null space analysis. In particular, spiked covariance leads to a narrower null space (after whitening) which reduces the sample complexity. Such narrow or modified null space analysis is closely related to the weighted compressed sensing literature which modifies $\ell_1$ minimization based on prior information regarding the nonzero support of the parameter \cite{khajehnejad2009weighted, vaswani2010modified,oymak2012recovery,mansour2017recovery,xu2010breaking}.

Our main result of this section demonstrates that such improved sample complexity bounds persist with much more general covariance matrices which connects our discussion to Section \ref{sec grad cov select}. Specifically, we prove that the benefits of spectral bias is persistent for covariance matrices that contain arbitrarily large low-rank components.

\begin{theorem}[Sample bounds for general covariance]\label{cov gen thm} Fix condition number $\kappa\geq 1$ and rank $d\geq 0$. Let $\bSi_{LR}\succeq 0$ be a rank $d$ matrix and $\bSi_{\text{tail}}\succeq 0$ satisfy $\Iden_p\succeq \bSi_{\text{tail}}\succeq \kappa^{-1}\Iden_p$. Suppose the samples $(\x_i)_{i=1}^n\distas\Nn(0,\bSi)$ have the covariance
\[
\bSi=\frac{R-1}{s}\s\s^T+\bSi_{LR}+\bSi_{\text{tail}}.
\]
If $\sqrt{n}\geq \sqrt{d}+\sqrt{\kappa s(\frac{3}{2}+\frac{2\log(p/s)}{R^2})}+t$, with probability at least $1-\exp(-t^2/2)$, $\bt_\st$ is the unique solution of \eqref{l1 prob}.
\end{theorem}
This result characterizes the required sample complexity in terms of sparsity $s$, condition number $\kappa$, bias $R$ and principal subspace rank $d$. The key message is that sample size bounds of Lemma \ref{thm spike} is robust to the changes in the condition number (suffers a multiplicative term of $\kappa$) and {\em{arbitrarily large}} low-rank perturbations on the covariance matrix (suffers an additive term $d$).
%to encourage   conditionapplying whitening, it can be shown that $\omega_R(\Tc)\leq\omega(\Tc_R)$ where $\omega(\cdot)$ is the usual Gaussian width with identity covariance and $\Tc_R$ is the set
%\[
%\]

% the covariance, null space condition associated with $\omega_R
% regression problem over this dataset. 
%$\xb_i\sim\Nn(0,\Iden_p)$

